The Completed SDSS-IV extended Baryon Oscillation Spectroscopic Survey: A Catalogue of Strong Galaxy-Galaxy Lens Candidates

We spectroscopically detected 838 likely, 448 probable, and 265 possible strong lens candidates within $\approx2$ million galaxy spectra contained within the extended Baryon Oscillation Spectroscopic Survey (eBOSS) from the sixteenth data release (DR16) of the Sloan Digital Sky Survey (SDSS). We apply the spectroscopic detection method of the Baryon Oscillation Spectroscopic Survey (BOSS) Emission-Line Lens Survey (BELLS) and add Gaussian fit information, grading, additional inspection observables, and additional inspection methods to improve our selection method. We observed 477 candidates with lensing evidence within low-resolution images from both the Legacy survey of SDSS-I/II and the DESI Legacy survey, which is $12\%$ higher than the percentage of BELLS candidates observed with similar lensing evidence. Our search within the latest and improved reductions of the BOSS survey yielded a $20\%$ increase in the number of lens candidates expected from searching all BOSS and eBOSS galaxies. The distribution of target and background redshifts of our candidates is similar to the candidates and confirmed lenses within the BELLS observations. We present our Spectroscopic Identification of Lensing Objects (SILO) candidates in a value-added catalogue (VAC) in SDSS DR16. The examination of these lens candidates in follow-up high-resolution imaging may yield more than twice the lenses found in previous spectroscopic detection surveys within SDSS, which would extend the results of previous lens surveys within SDSS to higher redshifts, constrain models of mass structures in spiral galaxies, and test if including the identification of possible lensing features within low-resolution images has merit to spectroscopic detection programs.

==> tex/database_code_and_results.tex <==
checks in paper

check adding histogram to vac!!! (so since passed hist changes)
CHECK if re-write acknolegements!!!!!!!!!!!!!
check assumption of test einstein radius of mass reduction
MAKE SURE IMAGE EXAMPLES ARE NAME EQUALS IMAGE(likely so since i do not remember editing the paths to the images, and thus neither the associated names)

check quo for source type
refine via 450 kpc does not seem to work right, check!!!!

look at hits around 4010 55350 610 even if grade x
6147 56239 4 shows where o3 model looks way off xposition!!!!!!!!!!!!!!!!!!!!!!!!!!! (more than one example!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!) (the model is correct but the window is not exactly directly on…poss for setting window xrange. notice arrow over hit)
1.073 can have fake 4Nline!!!!, though mostly weak

===>add wiki comment on flux images
===>add wiki comment on system name

CHECK:
2. Target emlines vs absorption (seems rather verified that these are emission lines)
3. image not blure due to atmospheric seeing (images consistant across decals and sdss in same orientation, thus not temp atmosphere, and about 1 in 5 of blue arc candidates show another poss blue nearby, but not on same side of target as candidates, so likely not DAR
6. should we change to gauss fwhm vs unvariatespline (mabey not since OII doublet spacing)
8. why *.7 in 74 of spectrum for gaus width (basically matches bounds of 8)
9. The wave window of 8.4 (see above) might be too small for high redshift targets for eboss and BOSS…consider widening since current pixel plus z expaned doublet is 9.87 (adjusted to sigma pixel scale instead)
10. RUN GAUSSFIT and GAUSSCOMPARE!!!!!!! (did so…but check)
11. rerun images with correct scale!!!!!!! (do when at end of 
12. check filtering out known artifacts

NOTE: found where ivar_new may not be skymasked IF tries pass an hour!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!


===>GAUSS HEADER DATA IS OFFSET by 1 (i.e. OII header is H1b) Primary header was added to set each hit up one!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!
CHECK GAUSS IF OFFSET BY 1 bias left on wavelength for following wavelength of past OII
OII GAUSS spike dont vary enought (check vary amplitude option)!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!

he night sky emission lines at 5577Å, at 6300Å, 6363Å (when there is auroral activity), and in the OH forest in the red can be very strong, and leave significant residuals in the spectra whose amplitude is occasionally 

The sky spectrum estimates in BOSS (and in fact in SDSS) that are subtracted from each object are biased slightly low. This is due to the well-known bias associated with fitting an error-weighted model to data when the errors are estimated from the data itself (e.g. in the case of Poisson estimates of errors). These residuals can be detected by taking the average of the sky-subtracted sky fibers, which yield a slightly positive spectrum ranging from 7×10-20 erg/cm2/s/A at around 8000 Angstroms to up to 10-18 erg/cm2/s/A at the bluest and reddest end of the spectra.
5470 56008 599 304

Grade A- or higher with vi.s.
SDSS~J0032+2723 00:32:26.03 +27:23:04.51 A- o2.d,g.d,ml,o2.d,o3b.e,o3a.e,psc.o3b,h1.t.r.l.o3b,h1.t.l.h.o3a,psc.o3a,vi.s.n.d.d.s.A multiline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J0116+0011 01:16:01.72 +00:11:44.12 A+ o2.d,g.i,wh.o2,o3.f,ml,o2.d,o3b.f,o3a.f,wh.o3a,psc.o2,so.d.l,h1.s.c.l.o2,vi.s.n.d.d.s.A+ multiline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J0119+0101 01:19:49.19 +01:01:51.19 A o2.w,wh.o2,o3.d,ml,o2.w,o3b.d,o3a.f,psc.o2,so.r.m,psx,psc.o3b,psx,psc.o3a,psx,vi.s.d.f.d.A+ multiline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J0154+0141 01:54:38.94 +01:41:54.82 A o2.d,g.d,ml,o2.d,o3b.e,o3a.d,psc.o2,so.l.m,so.c.l,psc.o3a,vi.s.n.e.d.A+ multiline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J0159+1855 01:59:54.58 +18:55:41.52 A o2.f,g.d,ml,o2.f,hd.e,psc.o2,so.d.l,psx,vi.s.a.e.d.s.A+ multiline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J0204+0210 02:04:42.97 +02:10:55.49 A+ o2.d,g.d,ml,o2.d,hc.e,hb.d,o3a.d,wh.o3a,pte.o2.FeVII,jedw,h1.t.c.l.o2,psc.hc,psc.hb,psx,pte.hb.SII,psc.o3a,psx,vi.s.d.e.d.s.A+ multiline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J0213-0347 02:13:00.49 -03:47:03.10 A+ o2.f,g.d,wh.o2,o3.f,ml,o2.f,hd.e,hc.e,hb.f,o3b.f,o3a.f,wh.o3a,psc.o2,so.l.l,psx,h1.t.l.m.o2,psc.hd,so.d.l,psx,psc.hc,so.l.l,psx,vi.s.a.d.d.s.A+ multiline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J0731+3635 07:31:52.65 +36:35:21.19 A- o2.w,g.i,ml,o2.w,hb.e,o3a.f,psc.o2,so.c.h,so.l.l,vi.s.d.e.m.A multiline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J0737+1914 07:37:09.51 +19:14:35.84 A+ o2.f,g.d,o2.f,hb.e,psc.o2,so.c.l,vi.s.ma.e.d.s.A+ multiline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J0743+3208 07:43:02.60 +32:08:32.15 A+ o2.f,g.d,wh.o2,o3.f,ml,o2.f,hd.e,hc.d,hb.f,o3b.f,wh.o3b,o3a.f,wh.o3a,psc.o2,so.c.l,h1.s.r.h.o2,h1.t.l.h.o2,psc.hd,psx,psc.hc,psx,psc.hb,psx,psc.o3b,psx,psc.o3a,psx,vi.s.a.d.d.m.s.A+ multiline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J0814+2318 08:14:32.90 +23:18:21.83 A o2.f,g.d,psc.o2,so.l.l,psx,vi.s.d.e.d.A+ multiline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J0830+1206 08:30:52.88 +12:06:56.35 A o2.d,g.d,o3.e,ml,o2.d,o3b.e,o3a.f,psc.o2,so.d.l,h1.t.c.h.o2,psc.o3b,psc.o3a,psx,vi.s.n.e.d.s.A+ multiline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J0832+0628 08:32:30.57 +06:28:26.30 A o2.w,g.s,o3.e,ml,o2.w,o3b.e,o3a.d,h1.t.l.h.o3b,h1.t.c.l.o3a,hst.t.r.h.o2,vi.s.a.e.d.s.A+ multiline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J0841+0811 08:41:43.46 +08:11:14.20 A+ o2.f,g.d,o3.d,ml,o2.f,hb.e,o3b.d,o3a.f,pte.o2.FeVI,jedw,psc.o2,so.c.m,psx,psc.hb,psx,h1.t.c.h.hb,h1.t.l.h.o3a,vi.s.ma.e.d.s.A+ multiline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J0846+5218 08:46:33.27 +52:18:13.61 A- o2.d,g.d,ml.o2.d,o3a.d,pte.o2.CaV,jedw,h1.t.r.h.o2,psc.o3a,psx,vi.s.n.d.m.s.A multiline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J0849+2202 08:49:07.24 +22:02:40.47 A+ o2.f,g.d,ml,o2.f,hb.e,psc.o2,so.d.l,vi.s.a.d.d.s.A+ multiline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J0851+0218 08:51:30.07 +02:18:23.24 A- o2.d,g.d,ml,o2.d,hc.e,psc.o2,so.r.h,so.l.m,lgwmw,vi.s.d.e.d.s.A- multiline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J0858+4145 08:58:58.56 +41:45:50.30 A- o2.d,g.d,pte.o2.FeVII,psc.o2,so.d.l,vi.s.a.d.m.s.A- multiline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J0911+5253 09:11:42.30 +52:53:20.73 A o2.d,g.d,ml.o2.d,hd.e,o3a.e,psc.o2,so.r.l,psx,psc.hd,h1.s.c.h.hd,psc.o3a,psx,h1.t.c.l.o3a,hst.t.c.h.o2,vi.s.n.d.m.s.A multiline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J0917+3109 09:17:26.81 +31:09:25.12 A+ o2.f,g.d,wh.o2,o3.f,ml,o2.f,hc.d,hb.e,o3b.d,o3a.f,wh.o3b,wh.o3a,psc.hb,vi.s.n.e.d.A+ multiline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J0917+4218 09:17:37.34 +42:18:18.63 A o2.f,g.d,ml,o2.f,o3a.e,h1.t.c.h.o3a,vi.s.d.e.m.s.A+ multiline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J0919+3103 09:19:30.05 +31:03:08.54 A+ o2.d,g.d,wh.o2,o3.d,ml,o2.d,hc.e,hb.d,o3b.d,o3a.f,psc.o2,so.r.l,psx,h1.t.l.h.o2,psc.hc,psx,psc.hb,psx,psc.o3a,psx,vi.s.d.d.d.A+ multiline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J0936+6032 09:36:36.97 +60:32:57.22 A o2.d,g.d,wh.o2,ml,o2.d,hb.d,o3a.d,psc.o2,so.r.l,psc.hb,psx,psc.o3a,psx,h1.t.c.h.o3a,vi.s.n.d.m.A+ multiline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J0942+0708 09:42:20.41 +07:08:34.83 A- o2.f,g.d,wh.o2,psc.o2,so.l.l,psx,hst.s.c.h.o2,vi.s.d.e.d.A multiline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J0955+3032 09:55:05.21 +30:32:30.57 A o2.f,g.d,wh.o2,ml,o2.f,hd.e,hc.e,hb.e,o3a.d,psc.o2,so.d.l,h1.s.c.l.o2,h1.t.r.l.hb,psc.o3a,psx,vi.s.d.d.d.m.s.A+ multiline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J0958+3745 09:58:24.53 +37:45:13.19 A- o3.f,ml,o3b.d,o3a.f,vi.s.d.e.m.s.A multiline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J1002+3035 10:02:20.23 +30:35:21.70 A+ o2.f,g.d,ml,o2.f,hb.d,psc.o2,so.d.l,psc.hb,psx,h1.t.r.h.hb,vi.s.n.e.d.s.A+ multiline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J1009+0131 10:09:12.73 +01:31:42.67 A+ o2.d,g.d,o3.f,ml,o2.d,o3b.f,o3a.f,psc.o2,so.c.l,so.l.m,psx,pte.o3a.NII,psc.o3a,psx,vi.s.a.e.d.s.A+ multiline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J1015+2127 10:15:37.19 +21:27:23.16 A o2.d,g.d,ml,o2.d,hb.e,o3b.e,o3a.d,psc.hb,h1.s.c.h.hb,psc.o3a,h1.s.l.h.o3b,h1.s.l.h.o3a,vi.s.n.f.d.s.A+ multiline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J1033+2612 10:33:08.69 +26:12:10.69 A+ o2.f,g.d,o3.f,ml,o2.f,hc.d,hb.f,o3b.d,o3a.f,pte.o2.FeIV,jedw,psc.o2,so.d.m,psx,psc.hb,psc.o3b,psc.o3a,psx,vi.s.a.e.d.s.A+ multiline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J1037+2956 10:37:31.60 +29:56:38.46 A+ o2.f,g.d,o3.f,ml,o2.f,hd.e,hc.d,hb.f,o3b.f,o3a.f,wh.o3a,psc.o2,so.c.l,psx,psc.hc,h1.t.c.m.hc,psc.hb,psx,psc.o3a,psx,vi.s.d.e.d.A+ multiline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J1043+4930 10:43:34.93 +49:30:01.94 A- o2.d,g.d,ml,o2.d,o3a.d,pte.o2.CiIII,jedw,psc.o2,so.c.l,so.r.h,so.l.h,vi.s.n.f.m.s.A,LITERAL:Potential nearby source starting to show arc indications but is at limit of expected strong lensing influence. multiline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J1051+4401 10:51:50.40 +44:01:42.47 A+ o2.f,g.d,wh.o2,o3.e,ml,o2.f,hd.e,hc.d,hb.d,o3b.e,o3a.e,psc.o2.so.d.l,psx,h1.t.c.h.hc,h1.t.c.h.hc,psc.o3b,psc.o3a,psx,vi.s.a.d.m.s.A+ multiline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J1057+4652 10:57:35.19 +46:52:31.73 A+ o2.d,g.i,o3.d,ml,o2.d,hc.e,hb.e,o3b.e,o3a.d,psc.o2,so.r.l,psx,psc.hc,pte.o3b.OII,psc.o3a,psx,vi.s.n.d.m.s.A+ multiline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J1105+5503 11:05:02.17 +55:03:09.02 A+ o2.f,g.d,wh.o2,psc.o2,so.l.m,f13,y2,vi.s.a.e.m.s.A+ multiline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J1112+0431 11:12:30.74 +04:31:53.30 A+ o2.f,g.d,wh.o2,ml,o2.f,hd.e,hc.d,hb.d,psc.o2,so.r.l,so.l.m,psx,y2,psc.hd,h1.s.r.h.hd,h1.t.l.h.hd,psc.hc,psx,psc.hb,psx,vi.s.d.e.d.s.A+ multiline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J1134+1712 11:34:27.96 +17:12:29.06 A+ o2.d,g.d,wh.o2,o3.d,ml,o2.d,hd.d,hc.e,hb.d,o3b.d,o3a.f,h1.t.c.m.o2,h1.s.l.m.o2,psc.hd,h1.t.r.h.hd,psc.hc,h1.s.r.h.hc,h1.s.c.h.hb,psc.o3b,psx,psc.o3a,psx,vi.s.a.e.d.s.A+ multiline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J1145+1022 11:45:59.88 +10:22:41.14 A+ o2.f,g.d,wh.o2,o3.f,ml,o2.f,o3a.f,wh.o3a,vi.s.n.d.d.s.A+ multiline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J1152+2753 11:52:55.24 +27:53:06.27 A o2.d,g.d,ml,o2.d,o3b.e,o3a.d,psc.o2,so.r.m,psx,h1.t.r.h.o3a,vi.s.a.d.d.s.A+ multiline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J1156+6623 11:56:24.00 +66:23:26.35 A+ o2.d,g.d,wh.o2,ml,o2.d,hd.e,hc.d,psc.o2,so.r.l,psx,psc.hd,psx,vi.s.n.d.m.s.A+ multiline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J1157+2627 11:57:54.31 +26:27:21.52 A o2.d,g.d,wh.o2,o3.e,ml,o2.d,o3b.d,o3a.f,y2,psc.o2,so.d.l,h1.s.c.m.o2,h1.t.c.l.o3b,vi.s.ma.e.d.s.A+,LITERAL:A nearby blue galaxy might also interfere with the signal, but is rejected as influential due to multiple emission lines at a redshift higher than the target. multiline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J1210+3149 12:10:24.00 +31:49:50.30 A+ o2.f,g.d,o3.d,ml,o2.f,hd.e,hb.e,o3b.d,o3a.f,psc.o2,so.d.l,psx,psc.hd,psx,vi.s.d.e.d.A+ multiline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J1215+4023 12:15:11.01 +40:23:18.61 A o2.d,g.i,ml,o2.d,hc.e,hb.d,psc.hb,psx,h1.t.l.h.hb,h1.t.c.m.o3a,hst.t.c.h.o2,vi.s.d.e.m.s.A multiline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J1216+0202 12:16:21.81 +02:02:35.72 A+ o2.d,g.s,wh.o2,o3.d,ml,o2.d,o3b.d,o3a.f,psc.o3b,psx,pte.o3a.HeI,vi.s.d.e.d.A+ multiline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J1235+4759 12:35:10.00 +47:59:14.14 A+ o2.f,g.d,o3.d,ml,o2.f,hb.d,o3b.e,o3a.d,psc.o2,so.r.m,psx,psc.o3a,psx,vi.s.n.d.m.A+ multiline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J1257+2946 12:57:39.36 +29:46:05.19 A o2.d,g.i,ml,o2.d,hb.d,psc.hb,psx,h1.t.r.h.hb,vi.s.n.d.d.A+ multiline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J1320+2403 13:20:33.31 +24:03:02.69 A o2.e,g.i,o3.e,ml,o2.e,hb.e,o3b.e,o3a.f,wh.o3a,pte.o2.FeIV,jedw,psc.hb,h1.s.l.h.hb,h1.t.l.h.hb,psc.o3b,psx,vi.s.n.e.d.s.A multiline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J1321+4018 13:21:26.22 +40:18:42.25 A+ o2.d,g.d,o3.d,ml,o2.d,hd.e,hc.d,hb.d,o3b.d,o3a.f,psc.o2,so.c.l,psc.hd,psc.hc,h1.t.c.m.hc,psc.o3b,psx,psc.o3a,psx,vi.s.n.f.m.s.A+ multiline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J1349+3612 13:49:10.30 +36:12:39.74 A+ o2.f,g.d,wh.o2,o3.d,ml,o2.f,hc.d,hb.f,o3b.e,o3a.f,pte.o2.FeIV,psc.o2,so.l.l,psx,psc.hc,psx,psc.o3b,psx,pte.o3b.FeII,psc.o3a,pte.o3a.NII,vi.s.n.e.m.s.A+ multiline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J1352+3216 13:52:18.99 +32:16:51.77 A+ o2.f,g.d,ml,o2.f,o3b.d,psc.o2,so.r.l,so.l.l,psx,psc.o3b,psx,vi.s.ma.e.d.m.s.A+ multiline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J1400+2116 14:00:03.04 +21:16:58.57 A+ o2.f,g.d,wh.o2,y2,o3.f,ml,o2.f,hd.d,hc.f,hb.d,o3b.f,wh.o3b,o3a.f,wh.o3a,h1.s.r.m.hd,h1.s.c.h.hc,psc.hb,psx,psc.o3a,psx,vi.s.d.e.d.A+ multiline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J1446+0439 14:46:02.08 +04:39:08.83 A o2.w,g.s,o3.d,ml,o2.w,o3b.d,o3a.f,psc.o3b,psx,vi.s.d.e.d.s.A+ multiline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J1503+0017 15:03:15.93 +00:17:31.67 A- o2.f,g.d,ml,o2.f,hb.e,pte.o2.FeV,jedw,psc.o2,so.d.l,psc.hd,vi.s.d.d.d.s.A multiline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J1503+0112 15:03:52.42 +01:12:04.36 A- o2.f,ml,o2.f,o3a.d,psc.o2,so.d.m,psc.o3a,psx,vi.s.d.e.d.s.A+ multiline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J1510+1902 15:10:21.10 +19:02:50.80 A o2.w,g.s,wh.o2,o3.e,ml,o2.w,hb.d,o3b.e,o3a.f,psc.o2,so.d.l,so.l.l,psc.hb,h1.t.l.h.hb,psc.o3b,vi.s.d.e.d.A multiline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J1547+5652 15:47:10.74 +56:52:52.02 A+ o2.d,g.d,wh.o2,o3.d,ml,o2.f,o3b.d,o3a.d,psc.o2,so.r.l,f2,psc.o3b,psx,psc.o3a,psx,vi.s.a.e.m.s.A+ multiline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J1600+4526 16:00:18.03 +45:26:46.20 A+ o2.f,g.d,wh.o2,y2,ml,o2.f,hc.d,hb.d,o3a.f,psc.hc,psc.o3a,vi.s.n.d.m.s.A+ multiline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J1602+3247 16:02:27.18 +32:47:54.07 A+ o2.f,g.d,wh.o2,o3.d,ml,o2.f,o3b.e,o3a.d,psc.o2,so.l.l,f13,h1.t.l.h.o2,psc.o3b,psc.o3a,vi.s.n.e.d.m.s.A+ multiline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J1611+0808 16:11:55.40 +08:08:20.82 A o2.d,g.d,ml,o2.d,o3a.d,h1.t.l.h.o3a,vi.s.d.e.d.A+ multiline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J1631+1854 16:31:50.33 +18:54:04.05 A+ o2.d,g.i,wh.o2,ml,o2.d,hc.e,hb.d,vi.s.a.e.d.s.A+ multiline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J1639+2625 16:39:39.12 +26:25:01.51 A+ o2.f,g.d,wh.o2,ml,o2.f,hd.e,hc.e,hb.d,o3a.f,pte.o2.CIV,jedw,psc.hc,psx,psc.hb,psx,psc.o3a,psx,vi.s.n.d.d.s.A+ multiline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J1710+2532 17:10:52.73 +25:32:48.42 A+ o2.f,g.d,wh.o2,o3.d,ml,o2.f,hc.d,o3b.e,o3a.f,psc.hc,vi.s.d.d.s.d.A+ multiline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J2210+1404 22:10:23.24 +14:04:57.05 A o2.d,g.i,ml,o2.d,hc.e,o3b.e,o3a.d,h1.s.r.h.hc,psc.o3b,vi.s.n.e.d.A multiline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J2227+0234 22:27:07.06 +02:34:59.86 A- o2.d,g.d,ml,o2.d,o3a.e,h1.t.l.l.o3a,vi.s.n.d.d.s.A+ multiline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J2239+2130 22:39:51.63 +21:30:53.05 A o2.w,g.s,wh.o2,ml,o2.w,hd.e,hc.f,wh.hc,hb.e,psc.o2,so.c.h,so.r.m,so.l.m,psx,vi.s.d.e.s.A+ multiline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J2310+1320 23:10:28.15 +13:20:02.14 A+ o2.f,g.d,wh.o2,y2,ml,o2.f,hc.d,pte.o2.ClIII,jedw,vi.s.d.e.d.s.A+ multiline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J2358-1030 23:58:59.76 -10:30:18.80 A- o2.d,g.d,psc.o2,so.d.l,vi.s.a.e.d.s.A multiline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J0018+1157 00:18:20.71 +11:57:57.36 A o2.f,g.d,psc.o2,so.l.l,psx,y2,vi.s.d.e.d.A+ oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J0024-0028 00:24:03.79 -00:28:32.22 A- o2.e,g.d,psc.o2,so.l.l,psx,y2,vi.s.d.d.d.A oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J0024-0133 00:24:05.90 -01:33:17.73 A- o2.d,g.d,ml,o2.d,hb.d,psc.o2,so.r.l,psx,vi.s.d.d.d.A oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J0029+2358 00:29:31.89 +23:58:33.36 A- o2.f,g.d,psc.o2,so.l.l,y2,so.c.l,vi.s.n.e.d.s.A oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J0030+3530 00:30:14.31 +35:30:09.10 A o2.d,g.d,y2,vi.s.d.e.s.A oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J0034+2653 00:34:46.50 +26:53:25.42 A+ o2.f,g.d,ml,o2.f,hc.d,y2,h1.t.r.l.o2,psc.hc,so.l.m,so.r.h,vi.s.n.e.d.s.A+ oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J0038+2100 00:38:07.58 +21:00:26.18 A o2.d,g.i,pte.o2.NiII,jedw,y2,vi.s.ma.f.d.s.A+ oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J0038+0103 00:38:26.81 +01:03:49.14 A o2.d,g.d,ml,o2.d,hb.e,psc.o2,so.r.l,psx,y2,vi.s.mi.e.d.s.A+,LITERAL:Second possible image appears in favor of discoloration instead of forming an indication of a shape. oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J0038+2940 00:38:57.92 +29:40:28.82 A o2.d,g.d,psc.o2,so.r.l,psx,vi.s.n.e.A oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J0106+0423 01:06:41.55 +04:23:22.72 A- o2.d,g.d,psc.o2,so.r.h,vi.s.r.d.d.s.A+ oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J0109+0352 01:09:50.73 +03:52:09.05 A o2.f,g.d,vi.s.d.e.d.s.A+ oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J0113+2830 01:13:19.01 +28:30:10.30 A- o2.d,g.d,psc.o2,so.r.m,psx,vi.s.d.e.d.s.A oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J0114-0229 01:14:31.33 -02:29:12.76 A- o2.d,g.d,psc.o2,so.l.m,psx,vi.s.a.d.d.s.A+ oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J0125+1026 01:25:32.29 +10:26:50.18 A o2.f,g.d,psc.o2,so.d.m,psx,y2,vi.s.n.d.d.s.A oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J0127-0406 01:27:20.03 -04:06:13.85 A+ o2.f,g.d,ml,o2.f,hc.d,psc.o2,so.r.m,so.l.h,psx,y2,vi.s.n.d.d.s.A+ oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J0130+0039 01:30:44.07 +00:39:07.78 A- o2.d,g.i,psc.o2,so.d.l,vi.s.d.e.d.s.A- oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J0138+0740 01:38:12.87 +07:40:23.56 A o2.f,g.d,pte.o2.SiII,jedw,vi.s.n.d.d.s.A+ oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J0141+0327 01:41:01.76 +03:27:41.97 A- o2.f,g.d,psc.o2,so.c.m,psx,vi.s.d.e.d.s.A oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J0148+3324 01:48:21.71 +33:24:18.76 A o2.d,g.d,psc.o2,so.l.m,psx,y2,vi.s.d.e.s.A oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J0157-0737 01:57:23.29 -07:37:55.53 A o2.f,g.d,psc.o2,so.l.m,psx,y2,vi.s.a.e.d.A+ oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J0208+0454 02:08:06.87 +04:54:51.52 A- o2.d,g.d,vi.s.n.d.d.s.A- oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J0210-0320 02:10:22.89 -03:20:21.59 A o2.f,g.d,y2,vi.s.a.e.d.s.A+ oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J0212+0300 02:12:16.12 +03:00:40.41 A o2.d,g.d,vi.s.d.e.d.s.A oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J0223-0553 02:23:23.09 -05:53:58.49 A o2.f,g.d,psc.o2,so.r.l,psx,vi.s.n.d.d.s.A,LITERAL:Nearby object might be overlapping. oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J0226+0110 02:26:07.42 +01:10:16.68 A+ o2.d,g.i,ml,o2.d,hc.d,o3a.d,psc.o2,so.r.m,f2,psc.hc,so.r.h,psc.o3a,so.c.h,h1.t.c.m.o3a,vi.s.d.e.d.A+,LITERAL:There are several other re-observations that show OII and OIIIa in most with possible OIIIb oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J0227-0113 02:27:38.60 -01:13:20.71 A o2.d,g.d,y2,vi.s.a.d.d.s.A+ oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J0259-0804 02:59:48.22 -08:04:46.33 A+ o2.f,g.d,wh.o2,psc.o2,so.l.h,psx,y2,vi.s.r.e.d.s.A+ oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J0717+4024 07:17:48.42 +40:24:51.00 A+ o2.f,g.d,wh.o2,psc.o2,so.c.l,so.r.l,psx,y2,vi.s.ma.d.m.s.A+ oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J0743+1554 07:43:32.45 +15:54:50.40 A- o2.d,g.d,ml,o2.d,hb.e,pte.o2.FeVI,jedw,psc.o2,so.l.l,psx,vi.s.n.f.d.s.A oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J0747+1939 07:47:53.11 +19:39:37.52 A o2.f,g.d,psc.o2,so.l.h,psx,h1.t.r.h.o2,vi.s.n.e.d.A+ oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J0749+2002 07:49:19.69 +20:02:37.05 A o2.f,g.d,y2,psc.o2,so.l.h,psx,vi.s.d.e.d.A+ oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J0757+0659 07:57:40.19 +06:59:47.36 A+ o2.f,g.d,psc.o2,so.r.h,h1.s.l.l.o2,vi.s.mi.e.d.s.A+ oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J0759+2422 07:59:41.00 +24:22:21.61 A- o2.d,g.d,psc.o2,so.l.l,so.r.h,psx,vi.s.d.e.d.s.A oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J0800+2402 08:00:00.23 +24:02:25.37 A o2.d,g.d,vi.s.n.e.d.s.A+ oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J0804-0029 08:04:41.29 -00:29:30.65 A o2.f,g.d,y2,vi.s.a.e.d.s.A+ oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J0806+3812 08:06:24.71 +38:12:11.64 A o2.d,wh.o2,psc.o2,so.c.l,y2,vi.s.d.e.m.s.A+ oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J0814+2208 08:14:49.01 +22:08:31.32 A o2.f,g.d,y2,psc.o2,so.c.l,psx,vi.s.d.e.d.A+ oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J0819+0225 08:19:30.46 +02:25:24.30 A o2.d,g.d,pte.o2.ClIII,jedw,vi.s.n.d.d.s.A+ oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J0823+2135 08:23:30.76 +21:35:12.07 A o2.d,g.d,vi.s.n.e.d.A+ oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J0834+3908 08:34:02.27 +39:08:48.68 A o2.f,g.d,psc.o2,so.d.l,so.c.l,psx,y2,vi.s.a.e.m.s.A+ oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J0839+0206 08:39:56.45 +02:06:32.40 A+ o2.f,g.d,wh.o2,vi.s.d.e.d.A+ oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J0840+5051 08:40:54.19 +50:51:53.14 A o2.d,g.d,wh.o2,y2,vi.s.d.e.m.A+ oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J0841+5017 08:41:21.74 +50:17:20.41 A o2.d,g.d,y2,vi.s.d.e.m.s.A+ oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J0843+4229 08:43:14.38 +42:29:15.41 A- o2.d,g.d,wh.o2,psc.o2,so.l.m,psx,y2,hst.t.c.m.o2,vi.s.n.d.m.s.A- oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J0844+1452 08:44:03.37 +14:52:35.78 A- o2.d,g.d,wh.o2,psc.o2,so.r.l,psx,y2,vi.s.a.e.d.s.A+ oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J0849+3508 08:49:36.13 +35:08:58.11 A- o2.f,g.d,ml,o2.f,hc.e,psc.o2,so.d.m,so.r.m,so.l.m,y2,vi.s.d.e.m.A oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J0900+3406 09:00:05.34 +34:06:00.45 A- o2.d,g.d,vi.s.n.e.d.m.A oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J0902+4745 09:02:19.35 +47:45:44.16 A o2.f,g.d,psc.o2,so.d.l,y2,vi.s.n.d.m.s.A+ oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J0903+2647 09:03:22.10 +26:47:45.14 A+ o2.d,g.d,wh.o2,psc.o2,so.l.m,psx,y2,vi.s.a.e.d.s.A+ oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J0923+4820 09:23:46.50 +48:20:19.68 A o2.f,g.d,psc.o2,so.d.l,psx,vi.s.n.e.m.A oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J0923+3206 09:23:58.21 +32:06:56.70 A+ o2.f,g.d,wh.o2,psc.o2,so.l.l,psx,h1.t.c.l.o2,vi.s.d.e.d.s.A+ oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J0925+1455 09:25:08.47 +14:55:51.26 A- o2.d,g.s,ml,o2.d,hb.e,o3a.e,psc.o2,so.d.l,so.l.l,psc.hb,so.r.m,psx,psc.o3a,so.c.l,vi.s.d.e.d.A- oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J0927+2839 09:27:24.38 +28:39:49.60 A- o2.d,g.d,pte.o2,jedw,h1.t.r.l.o2,vi.s.d.e.d.A oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J0927+3616 09:27:26.55 +36:16:47.81 A- o2.d,g.d,psc.o2,so.c.l,so.l.m,psx,y2,vi.s.n.e.m.s.A oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J0931+6353 09:31:22.57 +63:53:08.36 A- o2.f,g.d,psc.o2,so.l.h,psx,h1.t.l.h.o2,vi.s.d.e.m.s.A oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J0936+0824 09:36:22.14 +08:24:14.73 A o2.f,g.d,wh.o2,vi.s.a.e.d.s.A+ oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J0944+2910 09:44:13.36 +29:10:18.12 A o2.f,g.d,psc.o2,so.l.l,psx,vi.s.d.e.d.s.A+ oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J0946+2825 09:46:40.40 +28:25:20.37 A o2.d,g.d,ml,o2.d,hb.e,o3b.e,o3a.e,pte.o2.FeVI,jedw,psc.o2,so.d.l,psc.hb,so.d.l,psx,psc.o3a,so.r.h,h1.s.c.l.o3a,vi.s.d.f.d.s.A,LITERAL:Three different colors appear in the target image, in which the purple color does not seem related to the apparent mergers. oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J0947+3230 09:47:58.46 +32:30:00.95 A o2.f,g.d,vi.s.n.d.d.m.s.A+ oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J0957+3311 09:57:56.90 +33:11:51.98 A o2.f,g.d,psc.o2,so.d.l,psx,vi.s.a.d.d.m.s.A+ oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J1008+2153 10:08:44.74 +21:53:26.47 A+ o2.f,g.d,ml,o2.f,hb.e,o3a.d,psc.o2,so.c.l,psx,y2,psc.o3a,so.c.m,vi.s.a.d.d.s.A+ oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J1015+2449 10:15:35.02 +24:49:05.38 A- o2.d,g.i,psc.o2,so.r.l,psx,y2,vi.s.n.d.d.A oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J1016+1859 10:16:35.79 +18:59:49.38 A- o2.f,g.d,ml,o2.f,hd.e,hb.e,psc.o2,so.d.m,y2,psc.hd,so.d.m,psc.hb,so.c.l,vi.s.d.e.d.A+ oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J1016+2649 10:16:45.18 +26:49:16.05 A o2.f,psc.o2,so.r.m,psx,y2,vi.s.d.e.d.A oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J1017+0002 10:17:12.67 +00:02:41.61 A o2.f,g.d,ml,o2.f,hc.e,psc.o2,so.l.m,psx,y2,psc.hc,so.d.h,pte.hc.NI,vi.s.a.e.d.s.A+ oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J1020+4643 10:20:08.28 +46:43:32.89 A- o2.d,g.d,psc.o2,so.r.l,psx,y2,vi.s.n.f.m.s.A- oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J1021+0314 10:21:17.38 +03:14:42.10 A o2.d,g.d,y2,vi.s.d.e.d.s.A+ oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J1026+3705 10:26:53.64 +37:05:22.19 A- o2.f,g.d,psc.o2,so.l.l,psx,y2,pte.o2.FeVI,jedw,vi.s.d.e.m.A oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J1027+3729 10:27:35.64 +37:29:44.58 A+ o2.d,g.d,wh.o2,y2,vi.s.d.e.m.s.A+ oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J1032+3300 10:32:46.96 +33:00:23.33 A o2.d,g.d,psc.o2,so.d.l,vi.s.d.e.d.m.s.A+ oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J1035+3735 10:35:07.77 +37:35:11.83 A o2.d,g.d,psc.o2,so.r.l,so.l.l,psx,vi.s.n.f.m.s.A oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J1039+2629 10:39:35.65 +26:29:08.45 A o2.d,g.d,vi.s.d.e.d.A oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J1041+0359 10:41:59.33 +03:59:28.85 A- o2.d,g.d,y2,vi.s.n.f.d.s.A- oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J1044+4655 10:44:36.20 +46:55:01.66 A o2.d,g.d,y2,vi.s.d.e.m.A+ oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J1047+0016 10:47:01.03 +00:16:42.89 A o2.f,g.d,hst.t.c.l.o2,y2,vi.s.a.e.d.A+ oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J1050+2148 10:50:03.28 +21:48:32.85 A o2.f,g.d,ml,o2.f,hb.e,psc.hb,so.c.m,vi.s.n.d.d.s.A oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J1052+5905 10:52:13.43 +59:05:01.23 A+ o2.f,g.d,wh.o2,pte.o2.ClIII,jedw,y2,vi.s.d.e.m.A+ oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J1055+0846 10:55:56.35 +08:46:42.57 A- o2.d,g.d,psc.o2,so.d.m,psx,vi.s.d.e.d.A oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J1055+2611 10:55:59.80 +26:11:06.09 A o2.d,g.d,ml,o2.d,o3a.e,vi.s.d.d.d.s.A+ oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J1058+2904 10:58:36.81 +29:04:23.46 A+ o2.d,g.d,ml,o2.d,hb.d,vi.s.a.e.d.A+ oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J1102+2225 11:02:04.55 +22:25:05.39 A- o2.e,g.d,psc.o2,so.l.l,psx,y2,pte.o2.FeII,jedw,vi.s.a.e.d.A+ oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J1109+6704 11:09:09.01 +67:04:47.48 A o2.f,g.d,ml,o2.f,hd.d,hc.d,hb.d,psc.o2,so.c.l,so.l.l,f13,psc.hd,so.r.h,f13,psc.hc,so.l.h,psc.hb,so.l.h,so.r.h,psx,vi.s.n.d.m.s.A oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J1119-0206 11:19:35.42 -02:06:27.46 A o2.d,psc.o2,so.r.h,psx,vi.s.a.e.d.s.A+ oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J1126+0823 11:26:28.50 +08:23:27.99 A o2.d,g.d,psc.o2,so.r.l,psx,y2,vi.s.a.d.d.A+ oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J1129+4112 11:29:42.90 +41:12:58.66 A o2.f,g.d,pte.o2.FeVII,jedw,vi.s.mi.d.m.s.A+ oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J1129+4053 11:29:48.55 +40:53:18.97 A- o2.d,g.d,psc.o2,so.r.m,so.l.m,h1.s.l.l.o2,vi.s.d.e.m.s.A oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J1130+0536 11:30:30.82 +05:36:49.80 A+ o2.f,g.d,wh.o2,psc.o2,so.l.l,psx,y2,vi.s.a.d.d.s.A+ oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J1133+0133 11:33:08.13 +01:33:23.53 A- o2.d,g.d,psc.o2,so.c.l,so.r.l,psx,vi.s.n.d.d.s.A+ oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J1133+6002 11:33:28.68 +60:02:39.75 A o2.f,g.d,y2,vi.s.d.f.m.A,LITERAL:Red blob might be an overlapping object. oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J1139+4434 11:39:06.09 +44:34:49.74 A o2.f,g.d,psc.o2,so.l.m,so.r.m,vi.s.d.e.m.A oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J1141+5340 11:41:09.77 +53:40:58.52 A o2.d,g.d,o3.e,ml,o2.d,o3b.e,o3a.d,y2,h1.t.l.l.o2,hst.t.c.h.o3b,psc.o3b,so.r.l,psx,hst.t.c.h.o3a,psc.o3a,so.c.h,f13,vi.s.n.e.m.A oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J1145+3006 11:45:45.10 +30:06:44.79 A o2.d,g.i,wh.o2,y2,vi.s.d.e.d.s.A+ oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J1147+1919 11:47:56.14 +19:19:46.91 A+ o2.f,g.d,ml,o2.f,hc.f,psc.hc,so.r.h,f13,vi.s.d.e.d.A+ oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J1151+3035 11:51:04.02 +30:35:29.80 A o2.d,g.i,wh.o2,psc.o2,so.r.l,vi.s.n.d.d.m.A+ oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J1156+1255 11:56:17.74 +12:55:44.83 A o2.f,g.d,psc.o2,swmw,y2,vi.s.n.e.d.A oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J1156+2159 11:56:22.55 +21:59:16.70 A o2.e,g.d,psc.o2,so.l.h,psx,vi.s.q.f.d.s.A+ oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J1159+2431 11:59:32.84 +24:31:18.17 A o2.d,g.i,y2,wh.o2,ml,o2.d,hd.d,psc.o2,so.l.h,psx,psc.hd,so.c.h,vi.s.d.e.d.A+ oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J1202+3621 12:02:37.32 +36:21:32.85 A+ o2.f,g.d,psc.o2,so.d.l,psx,y2,hst.t.c.h.o2,vi.s.n.d.m.s.A+ oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J1202+1203 12:02:54.90 +12:03:51.50 A o2.f,g.d,wh.o2,ml,o2.f,hc.e,psc.o2,so.r.m,so.l.l,psx,y2,h1.t.c.h.hc,vi.s.ma.d.d.s.A+ oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J1209+3024 12:09:15.98 +30:24:51.51 A o2.f,g.d,wh.o2,psc.o2,so.l.l,psx,h1.t.r.h.o2,vi.s.d.e.d.s.A+ oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J1218+4546 12:18:07.52 +45:46:12.92 A- o2.f,g.d,psc.o2,so.c.l,so.l.l,psx,vi.s.d.e.m.s.A oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J1232+0601 12:32:38.08 +06:01:44.59 A- o2.e,g.i,ml,o2.e,hc.d,o3a.d,psc.o2,so.d.m,vi.s.a.e.d.s.A+ oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J1233+1407 12:33:20.16 +14:07:56.78 A o2.d,g.t,wh.o2,psc.o2,so.l.h,psx,y2,vi.s.ma.d.d.s.A+ oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J1236+4411 12:36:47.21 +44:11:42.21 A- o2.f,g.d,pte.o2.CLIII,jedw,vi.s.d.e.m.s.A oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J1240+1449 12:40:34.65 +14:49:03.41 A o2.f,g.d,psc.o2,so.c.l,psx,vi.s.d.e.d.A+ oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J1241+1102 12:41:45.96 +11:02:00.62 A o2.f,g.d,y2,h1.t.r.m.o2,vi.s.a.d.d.s.A+ oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J1249+0140 12:49:41.46 +01:40:50.11 A o2.f,g.d,psc.o2,so.l.m,psx,y2,vi.s.n.d.d.s.A+ oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J1258+0332 12:58:08.27 +03:32:08.73 A- o2.d,g.d,ml,o2.d,hd.e,pte.o2.FeII,jedw,psc.o2,so.c.l,so.l.m,psx,pte.hd.CIV,psc.hd,so.c.l,vi.s.a.d.d.s.A+ oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J1258+2917 12:58:31.27 +29:17:16.29 A- o2.d,g.i,vi.s.n.d.d.s.A oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J1258+1223 12:58:37.05 +12:23:35.51 A- o2.d,g.i,psc.o2,so.r.h,vi.s.d.d.d.s.A oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J1258+1010 12:58:45.74 +10:10:25.04 A+ o2.f,g.d,wh.o2,ml,o2.f,hc.e,psc.o2,so.r.l,so.l.l,vi.s.a.e.d.A+ oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J1308+0246 13:08:48.07 +02:46:02.91 A- o2.d,g.i,psc.o2,so.r.m,so.l.h,psx,vi.s.ma.e.d.s.A+ oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J1313+3630 13:13:04.32 +36:30:42.43 A+ o2.f,g.d,wp.o2,ml,o2.f,hc.e,psc.o2,so.r.l,y2,vi.s.n.d.m.s.A+ oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J1313+2616 13:13:32.17 +26:16:16.49 A- o2.d,g.i,skinny,y2,vi.s.n.e.d.A oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J1313+6004 13:13:55.85 +60:04:47.64 A o2.f,g.d,y2,vi.s.a.e.m.s.A+ oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J1313+1434 13:13:56.01 +14:34:23.47 A o2.f,g.d,psc.o2,so.r.h,psx,y2,vi.s.n.d.d.s.A+ oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J1318-0316 13:18:48.85 -03:16:03.66 A- o2.d,g.d,psc.o2,so.r.m,so.l.l,psx,y2,vi.s.d.e.d.s.A oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J1318+1237 13:18:53.09 +12:37:47.24 A+ o2.f,g.d,wh.o2,y2,vi.s.d.d.d.s.A+ oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J1321+2325 13:21:43.63 +23:25:15.42 A- o2.d,g.d,psc.o2,so.d.l,so.l.l,psx,vi.s.ma.e.d.s.A+ oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J1327+3725 13:27:44.04 +37:25:05.16 A o2.d,g.d,vi.s.d.e.m.s.A+ oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J1331+2202 13:31:34.46 +22:02:53.43 A o2.f,g.d,psc.o2,so.r.l,psx,vi.s.d.e.d.A oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J1338+0625 13:38:15.25 +06:25:38.59 A o2.d,g.d,vi.s.a.e.d.s.A+ oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J1343+2144 13:43:27.67 +21:44:19.42 A+ o2.f,psc.o2,so.d.l,psx,y2,vi.s.ma.e.d.A+ oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J1344+2709 13:44:28.47 +27:09:58.72 A- o2.d,g.d,skinny,vi.s.d.e.d.s.A oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J1345+0332 13:45:36.84 +03:32:40.11 A- o2.f,g.d,psc.o2,so.c.l,so.r.l,psx,h1.t.r.m.o2,vi.s.a.d.d.s.A+ oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J1347+0541 13:47:40.59 +05:41:16.08 A+ o2.f,g.d,wh.o2,ml,o2.f,hc.d,psc.o2,so.r.l,so.l.h,psx,vi.s.a.e.d.s.A+ oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J1349+1248 13:49:32.06 +12:48:15.39 A o2.f,g.d,psc.o2,so.l.m,psx,y2,vi.s.a.e.d.s.A+ oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J1350+5037 13:50:52.79 +50:37:39.99 A- o2.f,g.d,pte.o2.CIII,jedw,h1.t.r.l.o2,vi.s.d.e.m.s.A oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J1351+5207 13:51:31.94 +52:07:19.02 A+ o2.f,g.d,wh.o2,y2,ml,o2.f,hc.e,psc.hc,so.r.h,vi.s.ma.e.m.s.A+ oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J1352+2355 13:52:52.19 +23:55:12.86 A- o2.d,g.d,wh.o2,psc.o2,so.r.m,so.l.l,psx,pte.o2.FeIII,jedw,vi.s.d.e.d.s.A oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J1354+2500 13:54:37.18 +25:00:54.51 A+ o2.d,g.d,ml,o2.d,hd.e,hc.e,hb.d,o3a.d,psc.o2,so.d.l,psc.hd,so.r.m,psx,psc.hc,so.c.l,psc.hb,so.l.m,psc.o3a,vi.s.d.e.s.A+ oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J1358+1710 13:58:35.68 +17:10:27.50 A o2.f,g.d,wh.o2,pte.o2.FeIII,jedw,psc.o2,so.c.l,so.r.m,so.l.m,vi.s.d.e.s.A oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J1405-0022 14:05:37.00 -00:22:08.06 A o2.d,g.d,pte.o2.ClIII,jedw,vi.s.d.e.d.s.A+ oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J1412+2035 14:12:17.18 +20:35:29.34 A o2.w,g.s,wh.o2,ml,o2.w,hd.e,hc.d,vi.s.d.e.s.A+ oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J1414+3652 14:14:14.50 +36:52:37.52 A+ o2.f,g.d,wh.o2,ml,o2.f,hd.e,psc.o2,so.r.h,psx,y2,vi.s.a.e.m.s.A+ oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J1415+0901 14:15:42.16 +09:01:22.76 A o2.f,g.d,psc.o2,so.d.m,psx,pte.o2.FeVI,jedw,vi.s.ma.e.d.s.A+ oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J1416+4354 14:16:13.59 +43:54:08.58 A o2.d,g.d,psc.o2,so.r.l,psx,y2,vi.s.n.d.m.s.A oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J1416+3828 14:16:49.76 +38:28:55.50 A o2.f,g.d,o3.e,ml,o2.f,o3b.e,o3a.e,pte.o2.FeVII,jedw,hst.t.r.m.o2,vi.s.d.e.m.A+ oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J1421+5243 14:21:37.88 +52:43:00.92 A- o2.d,g.d,psc.o2,so.r.m,psx,vi.s.d.e.m.A oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J1424+3816 14:24:47.75 +38:16:30.06 A+ o2.f,g.d,psc.o2,so.l.h,psx,y2,vi.s.r.e.m.s.A+ oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J1428+2941 14:28:07.55 +29:41:30.83 A o2.f,g.d,y2,hst.t.c.h.o2,vi.s.d.e.d.A oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J1428+0318 14:28:22.46 +03:18:00.30 A- o2.d,g.d,psc.o2,so.l.l,psx,vi.s.a.f.d.s.A+ oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J1428+0058 14:28:40.13 +00:58:54.20 A+ o2.d,g.i,wh.o2,psc.o2,so.l.l,psx,y2,vi.s.d.e.d.A+ oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J1428+0828 14:28:40.95 +08:28:05.26 A o2.f,g.d,wh.o2,psc.o2,so.d.l,vi.s.d.e.d.A+ oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J1429+2716 14:29:51.72 +27:16:42.12 A o2.d,g.d,ml,o2.d,hb.d,sc.hb,so.c.h,vi.s.d.e.d.s.A+ oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J1436+2108 14:36:36.01 +21:08:42.96 A o2.f,g.d,wh.o2,psc.o2,so.d.l,so.r.l,psx,y2,vi.s.r.d.d.s.A+ oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J1436+1702 14:36:40.10 +17:02:37.31 A+ o2.f,g.d,wh.o2,psc.o2,so.l.h,psx,y2,vi.s.a.e.d.s.A+ oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J1440+0752 14:40:10.96 +07:52:53.56 A o2.d,g.d,vi.s.d.e.d.s.A+ oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J1441+3623 14:41:15.81 +36:23:16.85 A- o2.f,g.d,psc.o2,so.l.h,psx,vi.s.a.f.m.s.A+,LITERAL:Arc appears to be belong to an extended source. oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J1443+0702 14:43:54.17 +07:02:44.54 A o2.d,g.i,wh.o2,ml,o2.d,o3a.e,psc.o2,so.d.l,psx,h1.s.l.h.o3a,h1.t.r.h.o3a,vi.s.n.d.d.A oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J1451+3432 14:51:47.28 +34:32:09.91 A- o2.d,g.i,vi.s.a.e.m.s.A+ oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J1505+1715 15:05:35.60 +17:15:32.78 A+ o2.f,g.d,ml,o2.f,hd.d,hc.e,psc.o2,so.d.h,psx,psc.hd,so.c.m,psc.hc,so.l.h,vi.s.d.e.d.s.A+ oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J1508+3638 15:08:12.78 +36:38:38.38 A- o2.f,g.s,psc.o2,so.l.l,psx,pte.o2.FeII,jedw,vi.s.a.e.m.A+ oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J1515+0537 15:15:45.89 +05:37:04.25 A o2.d,g.i,wh.o2,psc.o2,so.l.l,psx,rs.f,vi.s.a.e.d.s.A+ oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J1520+0941 15:20:32.68 +09:41:08.12 A- o2.d,g.i,f4,f13,vi.s.d.e.d.A- oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J1523+3443 15:23:35.16 +34:43:37.61 A+ o2.f,g.d,wh.o2,y2,vi.s.n.d.m.s.A+ oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J1526+4117 15:26:51.90 +41:17:49.45 A- o2.f,g.d,pte.o2.FeVI,jedw,vi.s.n.e.m.A oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J1526+5603 15:26:53.59 +56:03:55.97 A o2.f,g.d,psc.o2,so.l.h,so.r.h,y2,vi.s.d.e.m.s.A+ oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J1529+1203 15:29:58.18 +12:03:28.07 A o2.f,g.i,ml,o2.f,hd.e,hc.e,pte.o2.FeXIV,jedw,psc.o2,so.r.l,psx,psc.hd,so.d.l,psc.hc,so.l.l,psx,vi.s.d.e.d.s.A+ oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J1532+2759 15:32:28.09 +27:59:23.16 A o2.f,psc.o2,so.l.h,so.r.m,psx,y2,vi.s.n.d.d.s.A oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J1532+5011 15:32:56.21 +50:11:43.23 A- o2.d,g.d,psc.o2,so.l.l,so.r.m,psx,y2,vi.s.d.e.m.s.A,LITERAL:Potential arc indications are positioned at a unrealistic distance. The latter is assumed to be one ore more nearby and unleansed galaxy or galaxies. oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J1534+0221 15:34:43.93 +02:21:25.65 A o2.f,g.d,psc.o2,so.r.h,so.l.m,psx,y2,vi.s.n.d.d.s.A oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J1541+1954 15:41:59.23 +19:54:52.87 A- o2.d,g.d,wh.o2,psc.o2,so.r.m,h1.s.c.l.o2,vi.s.d.e.d.A+ oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J1544+2610 15:44:02.70 +26:10:16.23 A- o2.d,g.i,wh.o2,psc.o2,so.r.h,so.c.h,so.l.h,vi.s.r.e.d.s.A+ oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J1547+0509 15:47:10.12 +05:09:37.73 A- o2.f,g.d,pte.o2.FeVI,jedw,psc.o2,so.d.l,psx,vi.s.n.e.d.A oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J1549+0605 15:49:04.31 +06:05:46.05 A- o2.f,g.d,psc.o2,so.l.h,psx,y2,vi.s.n.d.d.s.A+ oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J1555+4151 15:55:17.74 +41:51:38.63 A o2.f,g.d,psc.o2,so.l.h,so.r.m,psx,y2,vi.s.ma.d.m.s.A+ oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J1605+5413 16:05:00.30 +54:13:50.44 A- o2.d,g.d,psc.o2,so.l.l,so.c.l,pte.o2.FeXIV,jedw,vi.s.n.e.m.s.A oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J1611+3353 16:11:46.97 +33:53:55.20 A- o2.e,g.i,vi.s.d.e.d.m.s.A oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J1612+5414 16:12:09.16 +54:14:36.88 A- o2.d,g.d,psc.o2,so.r.l,vi.s.ma.e.m.A+ oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J1615+2056 16:15:23.55 +20:56:36.31 A o2.d,g.d,psc.o2,so.r.m,psx,vi.s.a.d.d.s.A+ oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J1615+1027 16:15:51.94 +10:27:57.33 A o2.d,g.d,psc.o2,so.r.h,psx,y2,pte.o2.FeVI,jedw,vi.s.d.e.d.A+ oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J1615+5324 16:15:59.65 +53:24:31.41 A- o2.f,g.d,psc.o2,so.l.l,psx,h1.t.r.m.o2,vi.s.r.e.m.A oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J1618+4620 16:18:12.13 +46:20:46.46 A- o2.f,g.d,pte.o2.FeIII,jedw,psc.o2,so.l.h,psx,vi.s.d.e.m.s.A oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J1622+5154 16:22:36.58 +51:54:37.84 A+ o2.f,g.d,wh.o2,psc.o2,so.d.l,psx,vi.s.n.e.m.s.A+ oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J1625+5552 16:25:46.47 +55:52:52.53 A+ o2.f,g.d,wh.o2,ml,o2.f,hd.d,hc.e,psc.o2,so.l.m,h1.s.l.l.o2,psc.hd,so.c.m,psc.hc,so.c.m,vi.s.r.d.m.s.A+ oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J1625+3310 16:25:50.96 +33:10:31.65 A+ o2.f,g.i,wh.o2,ml,o2.f,hc.d,psc.o2,so.r.l,psx,y2,rs.f,psc.hc,so.l.m,psx,vi.s.a.e.d.m.s.A+ oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J1639+1043 16:39:02.27 +10:43:55.82 A o2.d,g.d,psc.o2,so.l.l,psx,y2,vi.s.n.e.d.s.A+ oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J1654+2731 16:54:00.01 +27:31:20.79 A o2.f,g.d,ml,o2.f,hb.d,psc.hb,so.l.l,h1.s.c.h.hb,vi.s.a.e.d.s.A+ oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J1654+3643 16:54:31.74 +36:43:15.14 A- o2.d,g.d,pte.o2,psc.o2,so.r.m,psx,pte.o2.FeII,jedw,vi.s.d.e.m.A oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J1656+4003 16:56:03.88 +40:03:16.63 A o2.d,g.i,ml,o2.d,hc.d,psc.o2,so.r.l,psx,psc.hc,so.r.l,h1.s.l.h.hc,vi.s.a.d.m.s.A+ oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J1656+3705 16:56:55.10 +37:05:09.81 A o2.f,g.d,psc.o2,so.l.m,psx,y2,vi.s.d.e.m.A+ oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J1708+3427 17:08:21.39 +34:27:12.59 A o2.f,g.d,psc.o2,so.l.h,so.c.l,psx,y2,vi.s.d.e.m.A oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J1721+3707 17:21:17.20 +37:07:34.13 A- o2.d,g.d,psc.o2,so.r.m,so.l.h,psx,y2,vi.s.a.e.m.s.A+ oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J2122+0409 21:22:52.04 +04:09:35.53 A o2.f,g.d,vi.s.ma.e.d.s.A+ oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J2135-0139 21:35:04.97 -01:39:33.92 A+ o2.d,g.d,wh.o2,ml,o2.d,o3a.d,psc.o3a,so.d.l,psx,pte.o2.ArI,vi.s.d.e.d.A+ oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J2155+0655 21:55:34.77 +06:55:29.15 A o2.f,g.d,vi.s.d.e.d.s.A+ oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J2156+0359 21:56:39.90 +03:59:00.16 A o2.f,g.d,pte.o2.FeIV,jedw,vi.s.a.e.d.A+ oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J2219+1420 22:19:06.77 +14:20:52.41 A o2.f,g.d,pte.o2.CIV,jedw,psc.o2,so.r.l,psx,y2,vi.s.a.e.d.s.A+ oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J2238-0130 22:38:39.11 -01:30:29.18 A+ o2.d,g.i,ml,o2.d,hb.d,psc.o2,so.l.l,psx,pte.o2.FeVII,jedw,psc.hb,so.c.l,so.r.l,vi.s.d.d.d.A+ oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J2247+0614 22:47:15.00 +06:14:04.98 A+ o2.f,g.d,y2,vi.s.d.e.d.A+ oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J2249+0012 22:49:53.31 +00:12:20.38 A- o2.f,g.d,vi.s.d.d.d.A oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J2257+2531 22:57:56.06 +25:31:09.02 A- o2.d,g.d,psc.o2,so.d.l,swmw,vi.s.a.d.s.A+ oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J2300+0012 23:00:05.76 +00:12:06.37 A- o2.d,g.d,skinny,psc.o2,so.l.l,so.r.l,psx,y2,vi.s.n.e.d.s.A oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J2305+2704 23:05:38.29 +27:04:02.58 A+ o2.f,g.d,ml,hd.e,hc.e,psc.hd,so.r.l,psc.hd,so.d.m,vi.s.d.e.s.A+ oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J2312+0435 23:12:07.10 +04:35:01.83 A- o2.w,g.s,wh.o2,psc.o2,so.r.h,y2,vi.s.a.e.d.A oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J2331+2518 23:31:53.29 +25:18:59.14 A o2.d,g.t,wh.o2,ml,o2.d,hd.e,psc.o2,so.d.l,so.r.l,so.l.l,psx,y2,vi.s.a.e.d.s.A+ oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J2332-0030 23:32:40.53 -00:30:16.28 A+ o2.f,g.d,wh.o2,y2,vi.s.r.e.d.s.A+ oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J2333+1928 23:33:40.51 +19:28:39.34 A+ o2.f,g.d,vi.s.d.e.d.A+ oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J2344+1027 23:44:34.58 +10:27:17.15 A o2.f,vi.s.d.e.d.A+ oneline ACS WFCI CLEAR1L;F814W 8044.989
SDSS~J2358+0102 23:58:51.23 +01:02:23.50 A- o2.d,g.i,psc.o2,so.l.l,psx,pte.o2.FeVI,jedw,vi.s.d.e.d.A oneline ACS WFCI CLEAR1L;F814W 8044.989

NO HIT RANDOM 1000 SAMPLE COUNTS
counts {'r_f': 0, 'r_d': 0, 'r_e': 0, 'q_f': 0, 'q_d': 0, 'q_e': 0, 'ma_f': 0, 'ma_d': 0, 'ma_e': 0, 'mi_f': 0, 'mi_d': 0, 'mi_e': 0, 'a_f': 0, 'a_d': 4, 'a_e': 6, 'n_f': 2, 'n_d': 28, 'n_e': 13, 'd_f': 2, 'd_d': 4, 'd_e': 27}
fraction {'r_f': 0.0, 'r_d': 0.0, 'r_e': 0.0, 'q_f': 0.0, 'q_d': 0.0, 'q_e': 0.0, 'ma_f': 0.0, 'ma_d': 0.0, 'ma_e': 0.0, 'mi_f': 0.0, 'mi_d': 0.0, 'mi_e': 0.0, 'a_f': 0.0, 'a_d': 0.004, 'a_e': 0.006, 'n_f': 0.002, 'n_d': 0.028, 'n_e': 0.013, 'd_f': 0.002, 'd_d': 0.004, 'd_e': 0.027}
Percent {'r_f': 0.0, 'r_d': 0.0, 'r_e': 0.0, 'q_f': 0.0, 'q_d': 0.0, 'q_e': 0.0, 'ma_f': 0.0, 'ma_d': 0.0, 'ma_e': 0.0, 'mi_f': 0.0, 'mi_d': 0.0, 'mi_e': 0.0, 'a_f': 0.0, 'a_d': 0.4, 'a_e': 0.6, 'n_f': 0.2, 'n_d': 2.8000000000000003, 'n_e': 1.3, 'd_f': 0.2, 'd_d': 0.4, 'd_e': 2.7}


THE 10,000 any random galaxy!!!!!
counts {'r_f': 0, 'r_d': 3, 'r_e': 15, 'q_f': 0, 'q_d': 0, 'q_e': 0, 'ma_f': 0, 'ma_d': 1, 'ma_e': 3, 'mi_f': 0, 'mi_d': 2, 'mi_e': 2, 'a_f': 1, 'a_d': 25, 'a_e': 77, 'n_f': 17, 'n_d': 252, 'n_e': 312, 'd_f': 10, 'd_d': 51, 'd_e': 341}
fraction {'r_f': 0.0, 'r_d': 0.0003, 'r_e': 0.0015, 'q_f': 0.0, 'q_d': 0.0, 'q_e': 0.0, 'ma_f': 0.0, 'ma_d': 0.0001, 'ma_e': 0.0003, 'mi_f': 0.0, 'mi_d': 0.0002, 'mi_e': 0.0002, 'a_f': 0.0001, 'a_d': 0.0025, 'a_e': 0.0077, 'n_f': 0.0017, 'n_d': 0.0252, 'n_e': 0.0312, 'd_f': 0.001, 'd_d': 0.0051, 'd_e': 0.0341}
Percent {'r_f': 0.0, 'r_d': 0.03, 'r_e': 0.15, 'q_f': 0.0, 'q_d': 0.0, 'q_e': 0.0, 'ma_f': 0.0, 'ma_d': 0.01, 'ma_e': 0.03, 'mi_f': 0.0, 'mi_d': 0.02, 'mi_e': 0.02, 'a_f': 0.01, 'a_d': 0.25, 'a_e': 0.77, 'n_f': 0.16999999999999998, 'n_d': 2.52, 'n_e': 3.1199999999999997, 'd_f': 0.1, 'd_d': 0.51, 'd_e': 3.4099999999999997}


NA r_f
r_d 10.234052787244277
r_e 2.4561726689386263
NA mi_f
mi_d 13.539651837524177
mi_e 25.725338491295936
a_f 18.421295017039697
a_d 8.350987074391329
a_e 5.023989550101735
n_f 2.889614904633678
n_d 1.8275094262936207
n_e 0.9053200542562246
d_f 1.8421295017039696
d_d 3.1304161466864846
d_e 3.2052693187029


In [21]: fraction
Out[21]:
{'a_d': 0.0025,
 'a_e': 0.0077,
 'a_f': 0.0001,
 'd_d': 0.0051,
 'd_e': 0.0341,
 'd_f': 0.001,
 'ma_d': 0.0001,
 'ma_e': 0.0003,
 'ma_f': 0.0,
 'mi_d': 0.0002,
 'mi_e': 0.0002,
 'mi_f': 0.0,
 'n_d': 0.0252,
 'n_e': 0.0312,
 'n_f': 0.0017,
 'q_d': 0.0,
 'q_e': 0.0,
 'q_f': 0.0,
 'r_d': 0.0003,
 'r_e': 0.0015,
 'r_f': 0.0}

In [22]: counts
Out[22]:
{'a_d': 25,
 'a_e': 77,
 'a_f': 1,
 'd_d': 51,
 'd_e': 341,
 'd_f': 10,
 'ma_d': 1,
 'ma_e': 3,
 'ma_f': 0,
 'mi_d': 2,
 'mi_e': 2,
 'mi_f': 0,
 'n_d': 252,
 'n_e': 312,
 'n_f': 17,
 'q_d': 0,
 'q_e': 0,
 'q_f': 0,
 'r_d': 3,
 'r_e': 15,
 'r_f': 0}
 
 
 bells_grades
 10 14 3 2 1 3 1 0 1

[80 percent of BELLS candidates-half of those due to histograms and at least one due to difference in reduction identifier. Blind grading yields of BELLS of grade 77 percent or 4/5 had a grade of A like, 17 percent with B like and 1 confirmed C+ and 1 rejected C- like]

hit inspection ids to compare [(4174, 'A+', 'o2.f,g.d,ml,o2.f,hc.e,o3a.e,psc.o2,so.l.m,psc.o3a'), (4159, 'A', 'o2.d,g.d,wh.o2,ml,o2.d,hc.e,hb.e,o3a.d,psc.o2,so.l.l,psc.hb,psc.o3b,psc.o3a')]
[(4072, 'B', 'o2.e,g.s,wh.o2,ml,o2.e,o3a.d,psc.o2,so.l.m,so.r.h,psc.o3a'), (4190, 'B-', 'o2.d,g.i,psc.o2,so.l.l,LITERAL:Hint that OII is HIa of background.')]
[(3106, 'A+', 'o2.d,g.d,o3.d,ml,o2.d,hd.e,hc.d,hb.e,o3b.d,o3a.f'), (3544, 'A', 'o2.d,g.d,ml,o2.d,hc.e,o3a.d,pte.o2.FeVI,jedw')]
[(2260, 'B-', 'o2.d,g.s,psc.o2,so.r.l,vi.s.a.d.s.A-'), (2895, 'A-', 'o2.d,g.d,psc.o2,so.r.l,vi.s.a.e.s.A')]
[(2652, 'A-', 'o2.f,g.d,wh.o2,pte.o2.ClIII,psc.o2,so.r.l'), (2262, 'A', 'o2.d,g.d,psc.o2,so.r.h'), (2657, 'A', 'o2.f,g.d,wh.o2,pte.o2.ClIII,psc.o2,so.r.l')]
[(1716, 'B', 'o2.d,g.i'), (1358, 'C', 'o2.e,g.i,psc.o2,so.r.l,snde')]
[(577, 'A-', 'o2.d,g.i,psc.o2,so.l.l,pte.o2.FeVI'), (1088, 'B-', 'o2.d,g.d,wide,pte.o2.FeVI,jedw')]
NOTES FOR EBOSS VAC
OII flux and emline flux is not resflux!!!! consider removing!!!!!!
(NOT CORRECT ITS 43 from database or poss different from hit save check !!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!)54 for OIIIb to a is correct and ran on eboss, but verify in database correct since I might made this change after running(poss rerun gauss_compare for eboss)
DOUBLE CHECK THE chi and sig chi ect have recordings in eboss vac!!!!!!
HAVE astropy produce detailed SILO candidate name (with decimals) to convert to gal ra and dec for check but verify if specobj ra and dec dependent on time and if so update for year!!!!
check julian ra and dec the same for verifying previous hits!!!!!!!!!!! test on BELLS but note may not work the same if others julian is different!!!!!!
check via masterlens database since example ra converted not appear standard!!!!!!!!!!!!!!!
NOTE THAT NAMED DERIVED RA,DEC like in BELLS, but not bells gallery, are less accurate!!!!!!! Check master lenses as well
verify on next rerun that resflux at index 
check eboss emflux is resflux!!!! (vac now uses flux or resflux at index repectively for vac variables instead of hit emflux)
verify there is no gauss fails in vac below limit of spectrograph!! IF NOT....what about no signal situations!!!!!!!!!
check resflux, sky and model to flux is correct in vac since seems fishy
fix zerr_noqso since currently z in vac generation
I verified no zwarning > 0
I verified all selected class-noqso are galaxies
VAC NEES TO INCLUDE CLS... name and grade (currently not cls... despite noted) and other candidates from other papers!!!
[check update plot to include BELLS confirmed!!!]
[check plot is ratio per grade but REBIN to A, B, C and POSS get rid of C- that would fail if not for image, AND if undersampling of C multiline should be noted]
[double-check cited references are still right for this last iteration of intro]
[check different mjds and thus make sure rejecting duplicates and that paper stats are correct like vac!!!!!!]
[check update plot to show BOSS only candidates and the confirmed distribution of BELLS lenses]
[check remove Einstein radius from plot!!!!]
[check change to a more name-known statistical approach of math comparisons that accounts for different total counts in the sample since others I looked at did not do so].
[specify in new legend what is BELLS candidates vs BELLS confirmed]
[Perhpas INCLUDE BELLS CANDIDATES VS CONFIRMED]
[check any 'An extended catalog of galaxy-galaxy strong gravitational lenses discovered in DES using convolutional neural networks' and at least one or several 'Finding Strong Gravitational Lenses in the Kilo Degree Survey with Convolutional Neural Networks' and 'Survey of Gravitationally Lensed Objects in HSC Imaging (SuGOHI). II. Environments and Line-of-Sight Structure of Strong Gravitational Lens Galaxies to z ~ 0.8' and 'Survey of Gravitationally-lensed Objects in HSC Imaging (SuGOHI). I. Automatic search for galaxy-scale strong lenses']
The 17\% [check indications just for BOSS and not extended program] of lens candidates with indications of rings, multiple images, and arcs is the same percentage of indications of lensing found within the lens candidates of the BELLS GALLERY survey, despite this survey searched for lenses with Lyman-alpha emissions.
The LRG lenses found within the Legacy survey of SDSS-I/II [check I]
[check include biased towards high redshift for strong magnifiction or we just cannot confirm that now]
[check add image limit to optical depth]
[check if update acknowlegement or rewrite from MaNGA]
add OII to the signal to noise of the Gaussian fits
check left or right or centered histograms
poss switch mixed colors to Geometrically discernable variance in colors
check vs bells survey
check ratios of images per grade is not biased by counts present per grade



check blue
'3925', '55338', '570']
'5136', '55836', '608'
X 
A- '3615', '55445', '637'] (poss prior)

remove comma from '4039', '55648', '86']

reject visuals only?!!!!

blues never have nearby features

could the blue just be missed z quasar

Notes: Emergents might have some miss-identification chances when compared to 1 in several test of nearby squares (approx 1 in 3 quad search)
Non blue or purple hue showed 1 example nearby of several greys
Purple hue appears unique
Scroll down reveals not even fainter purple is spotted among a hundred object
Object arc purple is vary rare
Rarity of discernable (near emergent) purple arc is 1/1000 objects, which just suggest observed lenses
There are unique greys
random slight barely purple discoloration 1/200
full ring purple is not seen in environment around...not even hinted for at least 8 events
Purple hue almost definite!!
Nearly neon purple only hinted one possible emergent undependable in 50 searches
Blue and brown and grey can have nearby misshaps

Does flat appear to make a change (no on pits or rises or on any trend for elevation.)
Sky differences between coadd (no!)
unusual features confirmed (check but appears not-though some may have blue wings!!!!!!!!!!)
wdisp (no)
CR no
near skyline (appears common, check occurance of overlap!!!!!!!!!!!!!!!!)


cross check different nights and different flats!!!!!! 9578 57817 362


9341 57743 253 went low sigma to compensate for skinny walls. rchi 2.92
9597 58137 841 rchi2 not for o3b but is fitted (check NAN or INF messing chi up)
4024 55646 436 (cause is ivar not complete across flux)
4272 55509 991 o3b fit left and not as strong (cause is ivar not complete across flux)
6254 56268 385 might have arc or image smear
4553 55584 355 might have multi image

questions to ask in addition
include/exclude previous sightings
who column of previous surveys
Joel and adam on fits file credits (joel says yes, see if get Adam on vac in fits file)
28024
check ring comment of hit recorded about 4:20pm
 
CHECK rchi2 logic!!!!!!!!!!!!!!!!!!!!!!!!!!
sig fwhm or measured!!!!!!!!!!!!!!!!!!!!!
check comments
specprimary
update eboss catalog on production

check how many BELLS are in new
check spacing of OII
check consistency of detection sky notes at same z n same plate

3656-55241-167-3815

white o3a and b hit id
113481

bad hit
71127 mystery crash

check 
72444
67977

CHECK eboss_catalog_mv was not on bane or is correct!!!!!
1-801-483-6705

8. This is unlikely….but if I see the OII signal is more assuring in a specprimary = 0 reduction vs. a specprimary = 1 reduction of the same target, should I default to the reduction with specprimary == 1.


BELLS-I searched 239 plates with approx 500 successful galaxy redshift per plate = 119,500
which is 1 in 16.74 of galaxy spectra in BOSS + eBOSS

Which is 1 in 12.55 of galaxy spectra in BOSS

simple prediction is 13*45 = 585 candidates in BOSS, or 565 if 12.55 * 45
If nievly include eBOSS, will be 16.74*45=753 or 17*45=765


In [7]: onet = 0
   ...: multt=0
   ...: for grade in ['A+','A','A-','B+','B','B-','C+','C','C-']:
   ...:     print(grade, '&', Hit_inspection.query.join(Hit,Hit_inspection.hit_id == Hit.id).filter(Hit_inspection.grade == grade).filter(Hit.mode_id == 1).
   ...: count(), '&', Hit_inspection.query.join(Hit,Hit_inspection.hit_id == Hit.id).filter(Hit_inspection.grade == grade).filter(Hit.mode_id == 2).count(),
   ...:  r'\\')
   ...:     onet+=Hit_inspection.query.join(Hit,Hit_inspection.hit_id == Hit.id).filter(Hit_inspection.grade == grade).filter(Hit.mode_id == 2).count()
   ...:     multt += Hit_inspection.query.join(Hit,Hit_inspection.hit_id == Hit.id).filter(Hit_inspection.grade == grade).filter(Hit.mode_id == 1).count()
   ...: print(r'\hline')
   ...: print('Total &', multt, '&', onet, r'\\')
   ...:


from 11 to
172 emlines watched for (grabed from http://astronomy.nmsu.edu/drewski/tableofemissionlines.html who grabbed from http://www.nist.gov/pml/data/asd.cfm
, likely this citation Ralchenko, Yu., Kramida, A.E., Reader, J. and NIST ASD Team (2010). NIST Atomic Spectra Database (version 4.0), [Online]. Available: http://physics.nist.gov/asd [Tuesday, 20-Sep-2011 13:19:04 EDT]. National Institute of Standards and Technology, Gaithersburg, MD.)

  
  Extension: PRIMARY
SIMPLE True conforms to FITS standard
BITPIX 8 array data type
NAXIS 0 number of array dimensions
EXTEND True 
AUTHOR Michael Talbot Creator of detection file
INSP Michael Talbot Detection inspector
SOURCE SILO SILO
SILO_VER 1.0.1 1.0.1
RUN1D V5_13_0 Run1d version
RUN2D V5_13_0 Run2d version
RELEASE DR16 Release version
SAMPLING LOG Wavelength sampling type
SPECTRA COADDED Type of spectra used from eBOSS files
OIIB 3727.092 Restframe wavelength of OIIb
OIIA 3729.875 Restframe wavelength of OIIa
HID 4102.892 Restframe wavelength of HId
HIC 4341.684 Restframe wavelength of HIc
HIB 4862.683 Restframe wavelength of HIb
OIIIB 4960.295 Restframe wavelength of OIIIb
OIIIA 5008.239 Restframe wavelength of OIIIa
NIIB 6549.86 Restframe wavelength of NIIb
HIA 6564.614 Restframe wavelength of HIa
NIIA 6585.27 Restframe wavelength of NIIa
SIIB 6718.29 Restframe wavelength of SIIb
SIIA 6732.68 Restframe wavelength of SIIa
Extension: DETECTIONS
XTENSION BINTABLE binary table extension
BITPIX 8 array data type
NAXIS 2 number of array dimensions
NAXIS1 239 length of dimension 1
NAXIS2 1609 length of dimension 2
PCOUNT 296917720 number of group parameters
GCOUNT 1 number of groups
TFIELDS 31 number of table fields
Header and Table Data
RA Degree (1609) FLOAT Target right ascension
DEC Degree (1609) FLOAT Target declination
RA_HMS hour:':'' (1609) VARCHAR Target right ascension in hour:min:sec
DEC_DMS Degree:':'' (1609) VARCHAR Target declination in degree:min:sec
WAVE Angstroms (1609) VARIABLE_ARRAY_FLOAT Wavelength of spectra
FLUX 10^-17 erg/s/cm^2/Ang (1609) VARIABLE_ARRAY_FLOAT Coadded object flux
SKY 10^-17 erg/s/cm^2/Ang (1609) VARIABLE_ARRAY_FLOAT Coadded sky emissions
MODEL_SILO 10^-17 erg/s/cm^2/Ang (1609) VARIABLE_ARRAY_FLOAT Target model generated by SILO
RESIDUAL_FLUX 10^-17 erg/s/cm^2/Ang (1609) VARIABLE_ARRAY_FLOAT Residual flux of FLUX-MODEL_SILO
Extension: EMISSION_LINE_ANALYSIS
XTENSION BINTABLE binary table extension
BITPIX 8 array data type
NAXIS 2 number of array dimensions
NAXIS1 123 length of dimension 1
NAXIS2 6293 length of dimension 2
PCOUNT 1055364 number of group parameters
GCOUNT 1 number of groups
TFIELDS 24 number of table fields
Header and Table Data
EM_WAVE Angstroms (6293) FLOAT Wavelength of emission-line
FLUX_AT_INDEX 10^-17 erg/s/cm^2/Ang (6293) FLOAT Flux of emission-line(s) at INDEX
RESIDUAL_AT_INDEX 10^-17 erg/s/cm^2/Ang (6293) FLOAT Residual flux of emission-line(s) at INDEX
GAUSS_WAVE Angstroms (6293) VARIABLE_ARRAY_FLOAT Wavelength(s) center of Gaussian model
GAUSS_BASE_HEIGHT Angstroms (6293) FLOAT Gaussian model base height
GAUSS_AMPLITUDE Angstroms (6293) FLOAT Gaussian model amplitude
GAUSS_SIGMA Angstroms (6293) FLOAT Gaussian model sigma
GAUSS_FWHM Angstroms (6293) FLOAT Gaussian model derived full width at half maxim
MODEL_WAVE_BASE Angstroms (6293) VARIABLE_ARRAY_FLOAT Wavlength base of Gaussian model
GAUSS_MODEL 10^-17 erg/s/cm^2/Ang (6293) VARIABLE_ARRAY_FLOAT Gaussian model of residual flux
FITTED_RESIDUAL_FLUX 10^-17 erg/s/cm^2/Ang (6293) VARIABLE_ARRAY_FLOAT Residual flux segment used in Gaussian fit

visual in BELLS
[bells counts
mi 1 e
ma 2 e
a 1 d 1 e
n 1 e
d 3 e] comes to 20 percent with nearby or 18 percent without nearby

BELLS grade for visuals
Grade C 2
Grade B
‘’ 1
A 6

BELLS grade vs my grades for indications inspection
2 A for the two C
His A is my B- B A+ A
His ‘ ‘ is my A

737 BOSS detections in paper with grade above or equal to A-
1334 from BOSS and 216 from eBOSS

min of spectra resolution 2.3...
max of spectra resolution 3.4
mean of high OIIIa fwhm/(1+z) 2.867
median of high OIIIa fwhm/(1+z) 2.864
len of high OIIIa fwhm/(1+z) 11
std of high OIIIa fwhm/(1+z) .326
min of high OIIIa fwhm/(1+z) 2.283
max of high OIIIa fwhm/(1+z) 3.43

no divide by (1+z) (note these are 4 nlines or more)
max 6.655
min 4.524
std .708
mean 5.497
median 5.212

In [11]: c=300000

KMS peak velocity stats from sigma. CHECK USE ERROR WEIGHTED MEDIAN or MEAN!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!
In [12]: np.sqrt(3)*np.sqrt(2)*c*np.median(np.array(plot.hits.all())[:,6]/(np.array(plot.hits.all())[:,4]+1))/3728
Out[12]: 201.27432833021368

In [13]: np.sqrt(3)*np.sqrt(2)*c*np.percentile(np.array(plot.hits.all())[:,6]/(np.array(plot.hits.all())[:,4]+1),[10,90])/3728
Out[13]: array([147.74750590912782, 303.54974381663874], dtype=object)


References at a glance
options
H0 from time delays
	1964MNRAS.128..307R (proposal how to get H0)
	treu2013dark (more of a proposal)
	Kundi__1997 (SDSS lens)
	Suyu_2013 (blind analysis)
	Oguri_2007 (higher orders and some -mean of previous surveys)
	Chen_2019
	Wilson_2017
	Bonvin_2016
	Rathna_Kumar_2013
	Balm_s_2013
	Suyu_2010
	Kochanek_2001 (ER shape helps better get mass profile for time delay measurements)
    -Dark energy
	2012MNRAS.424.2864C (Collet to use double ER)
    -cosmological constant
	1990MNRAS.246P..24F
    -Flat
	Chiba_1997
    -Parameters of cosmology
	Mitchell_2005 (ΩΛ and Ωm)
Mass
	Allam_2007
    -profiles
	Wong_2017 (notes offset suggestive of offset from stellar, gas, and dust
	agnello2015high (constrained gamma)
	1995ApJ...445..559K (favors isothermals)
	1998ApJ...495..157K (halo, disk, bulge of spiral)
	2011MNRAS.417.1621D (trying to break spiral degeneracy of line above)
	2012MNRAS.424.2800L
	2012ApJ...752..163Sc (favors saltpeter and double ER constrains mean gamma)
	2015ApJ...803...71S (lower lens-galaxy masses reveal shallower higher velocity dispersions and larger DMF)
	Koo++09 (used SLACS ect to find results favoring isothermal and lots of other stuff)
    -DM
	Shu_2016 (mergers may show a candidate offset)
	Kochanek_2004 (Rules out alterative explanations of flux anamalies to leav low mass halos--check DM)
    -M/L
	2008ApJ...682..964B 
	Spiniello_2015 (includes bolton and is prep info)
	2009ApJ...705.1099A (check best here)
	2013ApJ...777...97S (lens and stellar mass-z up to .8 compliments SLACS)
    -statistical comparison to expected
    -substructures
	refId0 (simulations indicate flux-anomal properties)
	Vegetti09a (extended images to indicate DM subtructure)
	2010MNRAS.408.1969V (using double ER)
	2014MNRAS.442.2017V (11 but 10 not found)
	2016ApJ...823...37H (ALMA)
	2017arXiv170808854C(BELLS GALLERY surface-brightness profiles to use in dark-matter)
	2017arXiv171005029D (check DM but LOS haloes to test warm vs CDM)
    -lens model study
	Nightingale_2019 (red central from stellar envelope)
    -Time delay used to help constrain model
	Agnello_2017
    -With dynamics
	Koopmans_2006 (mass and z across gamma)
	2009MNRAS.399...21B (constrains allot from 6 SLACS lenses)
	2011MNRAS.417.3000S (compares Chambrier and Salpeter)
	2010ApJ...724..511A
	2012MNRAS.423.1073B (including Gaussian of image, compares Chambrier and Salpeter)
	2017ApJ...845..157N (Test stellar IMF)
     -Dark satellite galaxy
	2012Natur.481..341V
Source magnified
    -dwarf, lyman break, ect
	Poindexter_2008 (Quasar ecretion disk)
    -star formation
	Cabanac_2008(spectra)
	Bunker_2000 (find star formation knots)
    -galaxy formation
	Cui_2017 (no evolution of gamma per z)
	Cao_2016 (mild gamma per z)
	Li_2018 (study gamma per z)
	mukherjee2019seagleii(feedback)
	Oldham_2016 (red nuggets and where from)
	Capelo_2007 (explore how to extract properties of evolving galaxies)
	Marshall_2007(high redshift size-mass relation from -dwarfs)
    -Farther than available
	Fan_2019
	yamada1999emissionline (spectra)
	Hoag_2015(cluster)
    -supernovae in source
	Rubin_2018
    -Details better than available
	Johnson_2017(cluster)
	Brammer_2012(Image and spectra)
	Marques_Chaves_2018(Spectra)
	Smail_2006 (cluster-does not say if studied but delensed)
Cosmology
    -Test of cosmology simulations
	wang2017total (CDM for masses)
	Ritondale_2019 in tension with CDM, indicates sterile neutrino masses--
    -Distance scales
	Jee_2019(Lensing to convert 740 Ia from relative to absolute distances)
	de_Grijs_2017
	
Unsure
gilman2019constraints -mass-concentration relation on sub-galaxy scales
Nierenberg_2017 -seems to avoid broadband and looks at OIIIa to fit model to lensing features in order to test if a large mass was perturbing a certain lens, but ruled it out.
Sonnenfeld_2019-looking at discrepency of mass to stellar mass compared to mass models using lensing
benson2019normalization -semi simulate CDM haloes for sub-galactic scales and find slope results consistant, but they did not mention lensing in abstract while 1.9 to 1.8 indicate lens
10.1111/j.1365-2966.2005.09523.x -first pioneer of 'gravitational imaging' (i.e. mapping of luminous and dark matter within ER) to test distribution of CDM



Image search
Wong_2018
Brault_2015 (subtracts foreground but insufficient in lower resolution images)
Marshall_2009 (robot calibration on knowns)
10.1111/j.1365-2966.2008.12880.x (search for arcs)
Bom_2017 (test neural network arc finder)
Seidel_2007 (test on HST images of galaxy clusters to find pixels with arc connections)
Joseph_2014 (pca image subtraction and arc find)
Avestruz_2019 (HOG tested in simulations and dropped with efficiency for SLACS lenses)
Maturi_2014 (multi bands differences)
Gavazzi_2014 multi bands with 330 visual inspected candidates with 33 new GL confirmed (check if all imaged!!!!)
Ostrovski_2016 Gaussian mixture models with machine learning with multiple band imaging and spectrosopy to verify images and redshift
article neural network
huang2019finding -one of latest in DESI found 335 by training neural network

KEEP FOR REFERENCE COMMENTS
\begin{itemize}
\item Detect various types of distant galaxies~\citep{Allam_2007} and observe spacial and spectral features made possible because of the magnification boost from these cosmological telescopes~\citep{yamada1999emissionline (spectra of highest redshift luminous radio-quiet type-2 quasar), Bunker_2000 (cluster magnifies spectra for SF), Marshall_2007(examined the magnified source from cosmological telescope to size-mass expected from sersic, re, ect and found it ' source has the characteristics of the most compact faint blue galaxies studied and comparable size and mass to dwarf early-type galaxies in the local universe.'), Cabanac_2008 (stellar populations of g-g lyman break source), Poindexter_2008 (microlensing to see accretion disk in quasar), Brammer_2012 (examine low-metallicity star-bursting dwarf galaxy source from galaxy lens discovered from strong lensing Legacy survey), Oldham_2016(ELG-ELG lenses detected in SDSS spectra and study HST for clumpss, surface brightness,stellar mass and populations}. 
\item Use at least the position of the source images to either determine the mass enclosed within the Einstein radius\citep{Allam_2007(serendiputously discovered brightes lyman break known (in SDSS))} or fit a mass-density scale and profile for each lens in a sample to constrain the cosmological distribution of matter and galaxy formation models\citep{1995ApJ...445..559K(details of a radio lens distribution comparison to stellar dynamic models and galaxies modesl (like isothermal), 1998ApJ...509..561K (study 17 lenses across z.1to1 to find evolution and dark matter indicators and test dynamical and M/L models), 1998ApJ...495..157K(spiral study-apparently showing model simulations of halo, disk, and bulge to show occurance of hidden image by disk to suggest spirals not very flat, also compared some model to known spirals and propose more spiral lenses would provide usefull constraints on galactic structure), 2008ApJ...682..964B (SLACS V full sample and mass modeling to relate properties of ETG), 2008ApJ...684..248B (SLACS VII combine with sdss velocity dispersions to determening mass scale relations, including comparison to isothermal ect), 2009ApJ...705.1099A (slacs XI study of lens mass to lens light which also shows dm to light indications), Koo++09(fit SLACS lenses to slopes to determine isothermal homogenious models best fit), 2010ApJ...724..511A(slacs 10 uses velocity dispersions and stellar and surface photometry and strong lensing mass to determine allot of model parameters, DM ratio, hyperplane model usefull for galaxy formation models), 2011MNRAS.417.3000S(combine kinematic profile with gl and SDSS photometry to examine distribution and DM of a slacs lens to constrain saltpeter vs chabrier IMF and test to isothermal), 2012MNRAS.423.1073B (swells IV use kinematics and lensing and image of a lens to model a NFW dm profile and stell ar distributions as well as support chambrier over salpeter), 2012ApJ...744...41B(BELLS and measured pars of mass, light, ect), 2012MNRAS.424.2800L (model to constrain mass and light of a lens), 2013ApJ...777...97S(sonnenfield CFHT lenses used to measure mass model but more dependent on ER and images for surface and stellar masses of ETG), 2015ApJ...803...71S (s4tm lower mass lenses mass estimate), 2016ApJ...833..264S(bells galerry both lens mass and notice SF knots in magnified LAE), Cao_2016(constrain total mass profile across redshift to show evolving and support masses not mass follows light but DM fraction and SIS as effective model), Oldham_2016, Cui_2017(power law does not cosmologically evolve), Wong_2017 (ALMA mass for isothermal ect), 10.1093/mnras/stx2242(quasar), Li_2018(combine with dynamics to find total mass density profile out to 3er using SLACS and BELLS LENSES), mukherjee2019seagleii(compare to SLACS and BELLS lens simulations of comological with feedback models to constrain galaxy formation), Nightingale_2019(test Massive elliptcal models by using lensing to project stellar mass compared to visible mass--, Sonnenfeld_2019(fit lens with NFW to determine stellar mass-- vs mismatch to inferred by reference IMF)}, including using double sourced lenses to constrain the slope of the mass profile of the lens{}.
\item Combine lensing with dynamical measurements to dissect the stellar and dark matter distribution within one galaxy or a sample of galaxies across redshift (z)~\citep{Koopmans_2006(slacs lensing with dynamics to constrain gamma and evolution across z with no significant density slope evolution within 1re and dm fraction), 2009MNRAS.399...21B slacs lots of mass stuff with dynamics included and no evolution in redshift, 2010ApJ...724..511A, 2011MNRAS.417.1621D(combine dynamics to help break spiral disk+bulge+halow degereracy in a lens), 2011MNRAS.417.3000S, 2012MNRAS.423.1073B, 2017ApJ...845..157N(use lensing and dynamics to test consistancy of 3 nearest SIFONI lenses IMF)}, measure dark matter haloes perturbing the source light along the line-of-sight (LOS)~\citep{2017arXiv171005029D, Wong_2018}, or potentaily apply more sophisticated models to detect dark matter substructure within the lens~\citep{refId0(compare 17 quads with 4 actually focused on to simulations on how subtructure violates the zerod lensing signs of magnification when source near cusp and also expains more), Vegetti09a(baysean model to detect dm substructure but not compared to any lenses), 2010MNRAS.408.1969V(detected dm substructure in double lens), 2014MNRAS.442.2017V('Inference of the cold dark matter substructure mass function at z = 0.2 using strong gravitational lenses' in which only 1 in 11 lenses showed a luminous satellite, so they inferred the expected limits in substructure), 2016ApJ...823...37H(substructure hints using ALMA), 2017arXiv170808854C(morphology study of BELLS GALLERY Lya sources clumps reconstructed (de-lensed)), 2017arXiv171005029D(los vs substructure...los wins in contribution to perterbing ER shape)}.
\item Detect the gravitational influences of candidates dark satellite galaxy perturbing the mass distribution near the lens~\citep{2012Natur.481..341V (as described)}.
\item Examine repeated observations of flux-variant events in the source images to measure the Hubble expansion of the universe from the discrepancy between the variance in the arrival time of the source light and the time variance expected from the mass-density profile of the lens~\citep{1964MNRAS.128..307R(suggest possibility of time difference but no observation apparent), Kundi__1997 (galaxy-quasar H0), Kochanek_2001(ER galaxy-quasar small sample H0), Oguri_2007(comples lens potential model to better constrain 16 quasar sources for H0), Suyu_2010(constrain H0, spacial curvature, and dark energy equation of state from galaxy-galaxy), Balm_s_2013(two galaxy-quasar using Bayes for H0), Rathna_Kumar_2013(H0 fom quasar), Suyu_2013(H0 and cosmological parameters of galaxy-quasar), Bonvin_2016(H0 and cosmological parameters of 3 galaxy-quasar), Wilson_2017(testing how a sample of galaxy groups and environmental affect affect H0 in galaxy scale SGL sample not from SDSS), Chen_2019 (galaxy-quasar H0)}.
\item Constraining cosmological parameters to match the cosmological mass distribution~\citep{1990MNRAS.246P..24F(test without observations of constraining cosmological constant), Chiba_1997(statistically compares expected images separation statistic of qso images to 4 lenses for cosmological constant and apparent other pars to suggest flat univers), Mitchell_2005(lensing with sdss velocity dispersions to use apparently quasar CLASS sample to constrain two cosmological pars)}
\item Test the proposed types of dark matter~\citep{10.1111/j.1365-2966.2005.09523.x (test on artificial lens for gravitational imaging of luminous and dark matter substructures that can help provide insights into CDM), benson2019normalization(model expected slope and subhaloes that can be constrained in future work and was kinda tested to 6 galaxy-quasars apparently)}.
\item Use rare lenses with several sources to provide a probe into the dark energy equation of state which is independent of the Hubble expansion~\citep{2012MNRAS.424.2864C(mostly proposes this but forecast to 6 SLACS-made up double sources.)} and test gravity{}. 
\end{itemize}

Image detection surveys have tried, tested, and/or applied various methods to automatically identify lensing features at an angular radius beyond the flooding light of the lens~\citep{Seidel_2007 (arc finder tested on galaxy clusters), 10.1111/j.1365-2966.2008.12880.x(arc finder for DLS tested on simulates and present example candidates in DLS for galaxy-galaxy), Marshall_2009 (an automatic lens modeler simulated and tried on HST EGS high-resolution images and found 4 new lens candidates), Gavazzi_2014(ringfinder multiband imaging that filtered down to 330 candidates and 33 confirmed), Joseph_2014(pca subtraction of lens plus two arc finders...was lightly tested on real data), Maturi_2014(targets multi-color band selection of sources at z of about 1 and test on some data), Ostrovski_2016(machine learning with morphology source detection and found sourced quasar), Bom_2017(neural network arc finder simulated and HST tested), article(propose lensfinder neural network), Petrillo_2017, Wong_2018(YATTALENS searched images of galaxies in BOSS via HSC to find 41 definite or probable lens candidates), Avestruz_2019(lens searcher), huang2019finding(DESI nerual finding strong lenses)} and often beyond the solid angle covered by the single fiber surveys within SDSS, though some methods made some progress to observe past the foreground light to detect the source images~\cite{Brault_2015(tried to subtract lens to find candidates but test to CFHT 517 lens candidates showes subtracting foreground light the problem)}. Unlike the spectroscopic detection surveys, these imaging surveys often lack a significant set of confirmed lenses, which can make it difficult to assess the accuracy of each image detection method and train machine-learning methods. Follow-up imaging of the SILO candidates with indications of lensing in low-resolution images may provide a comparison to the efficiency/training/calibration information for low-resolution image searches within several arc-seconds of the target, such as searches within the DESI survey (Huang et al. (2019) and Wong et al. (2018)).


2009ApJ...705.1099A (slacs XI study of lens mass to lens light which also shows dm to light indications)
2013ApJ...777...97S(sonnenfield CFHT lenses used to measure mass model but more dependent on ER and images for surface and stellar masses of ETG)
1995ApJ...445..559K(details of a radio lens distribution comparison to stellar dynamic models and galaxies modesl (like isothermal)
2012ApJ...744...41B(BELLS and measured pars of mass, light, ect)

1998ApJ...495..157K(spiral study-apparently showing model simulations of halo, disk, and bulge to show occurrence of hidden image by disk to suggest spirals not very flat, also compared some model to known spirals and propose more spiral lenses would provide usefull constraints on galactic structure)

mass profile
2008ApJ...682..964B (SLACS V full sample and mass modeling to relate properties of ETG)
2015ApJ...803...71S (s4tm lower mass lenses mass estimate)
2016ApJ...833..264S(bells gallery both lens mass and notice SF knots in magnified LAE)
2012MNRAS.424.2800L (model to constrain mass and light of a lens)

indications of mass evolution across redshift
Cao_2016(constrain total mass profile across redshift to show evolving and support masses not mass follows light but DM fraction and SIS as effective model)
Cui_2017(theoretical power law does not cosmologically evolve--likely remove!!!!)
1998ApJ...509..561K (study 17 lenses across z.1to1 to find evolution and dark matter indicators and test dynamical and M/L models)

statistical inferrence of how galaxies formed
mukherjee2019seagleii(compare to SLACS and BELLS lens simulations of comological with feedback models to constrain galaxy formation)

compare to models
Koo++09(fit SLACS lenses to slopes to determine isothermal homogenious models best fit)
Wong_2017 (ALMA mass for isothermal ect)
Nightingale_2019(test Massive elliptcal models by using lensing to project stellar mass compared to visible mass--
Sonnenfeld_2019(fit lens with NFW to determine stellar mass-- vs mismatch to inferred by reference IMF)


==> tex/figures/stacked_OII.tex <==
\newcommand{\OIIstack}{Co-added Flux-Model of 831 candidate [O\,\textsc{ii}](b, a) doublets with a SN greater than 4 and a spectra grade of A- or above.}

\captionsetup{justification=centerfirst,hangindent=8pt,singlelinecheck=false,position=bottom,font={rm,md,up}}

\begin{figure}\setcounter{subfigure}{1}
\begin{center}
\label{figure.stackedOII}
\includegraphics[page=1, width=.35\textheight]{tex/figures/vac_plot_stack.pdf}
\end{center}
\caption{\OIIstack}
\end{figure}


==> tex/outline_and_coauthors.tex <==
eBOSS Detection
1.	Intro
a.	Use of lensing
i.	Cite use of Legacy lenses
ii.	Any summary-burning questions that can be answered with eBOSS?
b.	What has been found
i.	Previous surveys add up for the first million
ii.	Note difference between eBOSS and legacy
iii.	45 candidates from first 12th of BOSS in BELLS
c.	SILO extends search to eBOSS
i.	Note detection code nearly identical to BELLS
ii.	Summarize new refine and inspection tools
iii.	Overview of great results
d.	VAC overview for DR16 mini data release
e.	Paper outline
2.	Expectation
a.	Estimation
i.	Expected lenses to be found
b.	Simulation follows Arneston
i.	Expected lenses to be found 
3.	Data Used
a.	Spectroscopic detection
i.	eBOSS spectra
1.	Spectra from BOSS spectrograph
2.	Coadded
a.	Benefits to reject cosmic rays via sigma clip rejection
3.	Later reduction
ii.	NSA z for target z
iii.	Sky re-norm
iv.	Galaxy templates
b.	Inspection data
i.	Expand the library of aware potential target emission lines
ii.	Imaging
1.	SDSS
2.	DeCALS Legacy surveys (list 3 telescopes)
4.	Discovery
a.	Follows Bolton, Brownstein, ect
b.	Foreground subtraction
c.	SN detection
i.	Multi line
ii.	OII
iii.	Cound of detections
d.	Gauss-fitting
i.	MLE parallel best fit model
ii.	Use
1.	Model
2.	Rchi2 single to double Gaussian fit comparison for OII doublet as indicator
3.	FWHM check reasonable
4.	Amplitude ratios for OIII b,a
e.	Refine
i.	Summarize BELLS method
ii.	Note Einstein radius cut
iii.	Resultant detection count
f.	Inspection
i.	Spectra
1.	Signs of multiline signals
2.	Quality of signal
3.	Maskbit information
4.	Proximity to large library of target emlines
5.	Strong sky
6.	Occurrence of hit in sky or target emline locations
ii.	Low-resolution Images
1.	Supportive signs of multiple imaging, arcs, rings
2.	Signs of doubt casters such as nearby foreground galaxy
iii.	Candidates that remain
iv.	Example quad figure
v.	Table of detections????? (Check if this is too large)
5.	VAC
a.	Describe net count
i.	Figure of detection restframe to dz offset
b.	Describe catalog distribution of estimated ER
i.	Figure of ER distribution
c.	Resultant ratio of multiline to oneline due to higher end of spectrograph window
d.	Review VAC fits structure
i.	Table of VAC highlight values
6.	Conclusion


Candidate co-authors to request
From MaNGA paper
Adam S. Bolton
Kevin Bundy
Brett H. Andrews
Brian Cherinka
Thomas E. Collett
Anupreeta More
Surhud More
Alessandro Sonnenfeld
Simona Vegetti
David A. Wake
Anne-Marie Weijmans
Kyle B. Westfall

From BELLS paper
David J. Schlegel
Daniel J. Eisenstein
Christopher S. Kochanek
Natalia Connolly
Claudia Maraston
Parul Pandey
Stella Seitz
David A.Wake
W. Michael Wood-Vasey
Jon Brinkmann
Donald P. Schneider
Benjamin A. Weaver

For simulation
Arneston


==> tex/tables/apdx_vac_1_overflow.dat.tex <==
HIC &  4341.684 &  Angstroms & Float &  Restframe wavelength of HIc  \\
HIB &  4862.683 &  Angstroms & Float &  Restframe wavelength of HIb  \\
OIIIB &  4960.295 &  Angstroms & Float &  Restframe wavelength of OIIIb  \\
OIIIA &  5008.239 &  Angstroms & Float &  Restframe wavelength of OIIIa  \\
NIIB &  6549.86 &  Angstroms & Float &  Restframe wavelength of NIIb  \\
HIA &  6564.614 &  Angstroms & Float &  Restframe wavelength of HIa  \\
NIIA &  6585.27 &  Angstroms & Float &  Restframe wavelength of NIIa  \\
SIIB &  6718.29 &  Angstroms & Float &  Restframe wavelength of SIIb  \\
SIIA &  6732.68 &  Angstroms & Float &  Restframe wavelength of SIIa  \\

==> tex/tables/apdx_vac_2_overflow.dat.tex <==
WAVE & \AA & Float (Array) & Wavelength vector of spectra from BOSS/eBOSS \\
FLUX & \fluxunits & Float (Array) & Coadded object flux from BOSS/eBOSS \\
IVAR & & Float (Array) & Inverse varience of spectra from BOSS/eBOSS \\
AND\_MASK & & Integer (Array) & and\_mask of coadded spectra from BOSS/eBOSS \\
OR\_MASK & & Integer (Array) & or\_mask of coadded spectra from BOSS/eBOSS \\
SKY & \fluxunits & Float (Array) & Coadded sky emissions from BOSS/eBOSS \\
WDISP & \fluxunits & Float (Array) & Wavelength dispersion of spectra from BOSS/eBOSS \\
MODEL\_SILO & \fluxunits & Float (Array) & Foreground model generated by SILO  \\
IVAR\_RESCALED & & Float (Array) & Rescaled inverse varience  \\
RESIDUAL\_FLUX & \fluxunits & Float (Array) & Residual flux of FLUX-MODEL\_SILO  \\
SN\_SPECTRA\_SG & & Float (Array) & Gaussian convolved signal-to-noise of spectra \\
